A Short Course on Orthogonal Polynomials and Special Functions

These notes contain part of the lectures of an introductory course on orthogonal polynomials and special functions that I gave in the joint PhD Program in Mathematics UC|UP in the academic years 2015-2016 (at University of Porto) and 2016-2017 (at University of Coimbra). The notes were written for students who have never contacted with the above topics. Most results presented here can be found in the available bibliography at the end of each text/chapter, although in general more detailed proofs have been included (a few of them different from the ones presented in the source references), hoping this helps the beginner student.

==> opsf_appx2_2016-17.tex <==


\chapter{The Riemann-Stieltjes integral}\label{Appx2}

\pagestyle{myheadings}\markright{The Riemann-Stieltjes integral}
\pagestyle{myheadings}\markleft{J. Petronilho}

In this text we present a review on the Riemann-Stieltjes integral.
The material presented here is mainly from the classical book \ref{KolmogorovFomini1968-A2}
by A. Kolmogorov and S. Fomini.
For simplicity---and since it is enough for our purposes---we will introduce
the Riemann-Stieltjes integral with respect to a bounded nondecreasing and right-continuous function
on an interval of real numbers, but the construction is similar considering a function of bounded variation
(as a matter of fact, such a function may be written as a difference of two nondecreasing functions).

\section{Definition}

We start with two functions
$$
\phi:[a,b]\to\mathbb{R}\;,\qquad f:[a,b]\to\mathbb{R}\;,
$$
where we assume that $\phi$ is a bounded nondecreasing and right-continuous function.
The Riemann-Stieltjes integral of $f$ with respect to $\phi$ will be defined as an appropriate limit
of certain approximation sums, analogous to those used to define the ordinary Riemann integral.
Henceforth, let
\begin{equation}\label{PartitionP}
P\quad:\quad a=x_0<x_1<\cdots<x_{i-1}<x_i<\cdots<x_{n-1}<x_n=b\;,
\end{equation}
be a partition of the interval $[a,b]$. Choose $n$ arbitrary ``intermediate points''
\begin{equation}\label{PartitionQ}
\xi_i\in[x_{i-1},x_i]\;,\quad i=1,2,\ldots,n\;,
\end{equation}
and form the {\sl Riemann-Stieltjes sum} of $f$ with respect to the function $\phi$, subordinate to the partition $P$ and to the sequence of intermediate points $Q:=(\xi_1,\cdots,\xi_n)$:
\begin{snugshade}
\begin{equation}\label{RSsum-def}
\sigma_{\phi,P,Q}[f]:=\sum_{i=1}^nf(\xi_i)\big(\,\phi(x_i)-\phi(x_{i-1})\big)\;.
\end{equation}
\end{snugshade}
\noindent
Define also the diameter of the partition, $|P|$, as
$$
|P|:=\max_{1\leq i\leq n}\big|x_i-x_{i-1}\big|\;.
$$
Suppose that as the partition $P$ is ``refined''---i.e., as $|P|$ approaches zero---the sum (\ref{RSsum-def})
approaches a limit $L$, so that
\begin{snugshade}
\begin{equation}\label{RSsum-conv}
\lim_{|P|\to0}\sigma_{\phi,P,Q}[f]= L
\end{equation}
\end{snugshade}
\noindent
in such a way that $L$ is independent of the choice of both the points of subdivision, $x_i$, and of the
``intermediate points'', $\xi_i$. Then, $L$ is called the {\sl Riemann-Stieltjes integral of $f$ with respect to $\phi$} (or {\sl generated by $\phi$}), and it is denoted by
\begin{snugshade}
$$%\begin{equation}\label{RS-int-def}
\int_a^bf(x)\,{\rm d}\phi(x).
$$%\end{equation}
\end{snugshade}
\noindent
Moreover, if this integral exists, we say that $f$ is {\sl Riemann-Stieltjes integrable on} $[a,b]$.

\begin{remark}\label{RSremark1}\em
The precise meaning of the above limit (\ref{RSsum-conv}) is the following:
\begin{snugshade}
\begin{equation}\label{RSa1}
\forall\epsilon>0\;,\;\exists\delta>0\;:\;\forall P\in\wp[a,b]\;,\;\forall Q\in\Pi_P\;,\;
|P|<\delta\;\;\Rightarrow\;\;\big|\sigma_{\phi,P,Q}[f]-L\big|<\epsilon\;,
\end{equation}
\end{snugshade}
\noindent
where $\wp[a,b]$ is the set of all partitions of $[a,b]$ by points $x_0,x_1,\ldots,x_n$, as in (\ref{PartitionP}),
and $\Pi_P$ denotes the set of all the sequences $Q\equiv(\xi_1,\ldots,\xi_n)$ of $n$ ``intermediate points'' $\xi_i$ subordinate to the partition $P$, as in (\ref{PartitionQ}).
\end{remark}

\begin{remark}\label{RSremark2}\em
If $\phi(x):=x$, then the Riemann-Stieltjes integral reduces to the ordinary Riemann integral.
\end{remark}


\section{Basic properties}

As expected, many of the properties fulfilled by the Riemann-Stieltjes integral are obtained by transposition of the corresponding properties for the ordinary Riemann integral. For instance, the Riemann-Stieltjes integral is linear, i.e., the property
\begin{snugshade}
$$
\int_a^b\big(kf_1(x)+f_2(x)\big)\,{\rm d}\phi(x)=k\int_a^bf_1(x)\,{\rm d}\phi(x)+\int_a^bf_2(x)\,{\rm d}\phi(x)
$$
\end{snugshade}\noindent
holds, assuming that both $f_1$ and $f_2$ are Riemann-Stieltjes integrable functions with respect to $\phi$ on $[a,b]$,
and $k$ is a constant.
Also, being $\phi_1$ and $\phi_2$ bounded nondecreasing and right-continuous functions defined on the interval $[a,b]$, and $f$ a Riemann-Stieltjes integrable function with respect to $\phi_1$ and $\phi_2$ on $[a,b]$, then the equality
\begin{snugshade}
$$
\int_a^bf(x)\,{\rm d}\big(k\phi_1(x)+\phi_2(x)\big)=k\int_a^bf(x)\,{\rm d}\phi_1(x)+\int_a^bf(x)\,{\rm d}\phi_2(x)\;,
$$
\end{snugshade}\noindent
holds, where $k$ is a constant.
In bellow we list some important properties
under the assumption that $f:[a,b]\to\mathbb{R}$ is a continuous function.
This will be the most common situation over the course.

\begin{snugshade}
\begin{proposition}[properties of the Rieamann-Stieltjes integral]\label{propret-RSintegral}
Let $\phi$ be a bounded nondecreasing and right-continuous function
defined on the interval $[a,b]$, and let $f:[a,b]\to\mathbb{R}$ be a continuous function.
Then the following properties hold:
\begin{enumerate}
\item[{\rm (i)}] $f$ is Riemann-Stieltjes integrable with respect to $\phi$, and
the Riemann-Stieltjes and the Lebesgue-Stieltjes integrals of $f$ with respect to $\phi$ coincide.
\item[{\rm (ii)}] The following inequality holds:
$$\vspace*{-0.25em}
\Big|\int_a^bf(x)\,{\rm d}\phi(x)\Big|\leq\max_{a\leq x\leq b}|f(x)|\cdot\big(\phi(b)-\phi(a)\big)\; .
$$
\item[{\rm (iii)}] {\rm (Mean-Value Theorem)}
$$
\exists c\in[a,b]\;:\quad\int_a^bf(x)\,{\rm d}\phi(x)=f(c)\big(\phi(b)-\phi(a)\big)\; .
$$
\item[{\rm (iv)}] The Riemann-Stieltjes integral $$\int_a^bf(x)\,{\rm d}\phi(x)$$
does not depends on the values of the function $\phi$ at its points of discontinuity inside the interval $(a,b)$.
\item[{\rm (v)}] If $\phi$ is a step function with a finite or denumerable set of jumps
at the points $a_1,a_2,\ldots\in[a,b]$, being the jump at the point $a_j$ equal to
$$
h_j:=\phi(a_j+0)-\phi(a_j-0)>0 \quad (j=1,2,\ldots)\;,
$$
then
$$
\int_a^bf(x)\,{\rm d}\phi(x)=\sum_{j}f(a_j)h_j\; .
$$
%provided, whenever the number of jumps is an infinite (denumerable) set,
%the series on the right-hand side converges.
\item[{\rm (vi)}] If $\phi$ is an absolutely continuous function on $[a,b]$, so that
$\phi'(x)=w(x)$ exists a.e. for $x\in[a,b]$,
where $w$ is a Lebesgue integrable function on $[a,b]$, then
$$
\int_a^bf(x)\,{\rm d}\phi(x)=\int_a^bf(x)w(x)\,{\rm d}x\; ,
$$
where the integral on the right-hand side is a Lebesgue integral
(with respect to the Lebesgue measure),
which can be interpreted as an ordinary Riemann integral whenever
$w$ is Riemann integrable on $[a,b]$.
\end{enumerate}
\end{proposition}
\end{snugshade}

\begin{remark}\em
A {\it step function} $\phi:[a,b]\to\mathbb{R}$ as in property (v) is defined by
\begin{snugshade}
$$\vspace*{-0.25em}
\phi(x):=\sum_{\{j\in\mathbb{N}\,:\,a_j\leq x\}} h_j\;,
$$
\end{snugshade}\noindent
where $a_j<a_{j+1}$ and $h_j>0$ for each $j$, provided $\sum_{j} h_j<\infty$.
Notice that this function is indeed bounded nondecreasing and right-continuous.
Moreover, it is continuous at any point $x$ which does not coincide with any of the jump points $a_j$.
\end{remark}

\begin{remark}\em
An {\it absolutely continuous function} $\phi:[a,b]\to\mathbb{R}$ may be characterized as a function which
can be written in the form
\begin{snugshade}
$$
\phi(x)=\int_a^xw(t)\,{\rm d}t\;,\quad x\in[a,b]\; ,
$$
\end{snugshade}\noindent
where $w$ is a Lebesgue integrable function, being also the integral in the Lebesgue sense.
Often, $w$ is called a {\sl weight function}. For details on this subject,
%see e.g. the classical book \ref{KolmogorovFomini1968-A2} by A. N. Kolmogorov and S. V. Fomin,
see e.g. \ref{KolmogorovFomini1968-A2} or the more recent book by G. Leoni \ref{Leoni2009-A2}.
\end{remark}

\begin{remark}\em
The concept of Riemann-Stieltjes integral can be introduced also for a bounded nondecreasing and right-continuous function $\phi$ defined on an unbounded interval, as a natural extension of the ordinary Riemann integral. For instance,
\begin{snugshade}
\begin{equation}\label{RS-infty}
\int_{-\infty}^{+\infty}f(x)\,{\rm d}\phi(x):=
\lim_{a\to-\infty}\int_a^cf(x)\,{\rm d}\phi(x)+\lim_{b\to+\infty}\int_c^bf(x)\,{\rm d}\phi(x)\;,
\end{equation}
\end{snugshade}
\noindent
being $c\in\mathbb{R}$ arbitrarily fixed, provided all the Riemann-Stieltjes integrals
$\int_a^cf(x)\,{\rm d}\phi(x)$ and $\int_c^bf(x)\,{\rm d}\phi(x)$ exist for every $a,b\in\mathbb{R}$, with $a<c<b$,
and both limits appearing on the right-hand side of (\ref{RS-infty}) exist (finite).
\end{remark}

\medskip

\section*{Bibliography}
\medskip

{\small
\begin{enumerate}[label=\emph{\rm [\arabic*]},leftmargin=*]
\item\label{KolmogorovFomini1968-A2} A. Kolmogorov and S. Fomini, {\sl Introductory Real Analysis}, Dover Publications, Inc. (1975).
\item\label{Leoni2009-A2} G. Leoni, {\sl A first course in Sobolev spaces}, Graduate Studies in Mathematics, AMS, {\bf 105}
(2009).
\end{enumerate}
}



==> opsf_appx3_2016-17.tex <==


\chapter{Borel measures and the Lebesgue-Stieltjes integral}\label{Appx3}

\pagestyle{myheadings}\markright{Positive Borel measures and the Lebesgue-Stieltjes integral}
\pagestyle{myheadings}\markleft{J. Petronilho}

In this text we give a brief review on measure and integration theory,
including the Lebesgue-Stieltjes integral and its connection with the Riemann-Stieltjes integral.
The topics presented here are mainly from the classical book \ref{KolmogorovFumini1968-A2}
by A. Kolmogorov and S. Fomini, and from the \emph{online} notes by J. R. Norris (Cambridge) on Probability and Measure.

\section{Borel measures}

\begin{snugshade}
\begin{definition}\label{Borel-measure}
Let $X\equiv(X,\tau)$ be a topological space.
\begin{enumerate}
\item[{\rm (i)}]
The {\sl Borel $\sigma-$algebra} of $X$, denoted by $\mathfrak{B}_X$, is the
$\sigma-$algebra generated by $\tau$ (i.e., it is the smallest
$\sigma-$algebra in $X$ containing all the open sets in $X$).
\item[{\rm (ii)}]
A measure $\mu$ on $\big(X,\mathfrak{B}_X\big)$ is called a (positive) {\sl Borel measure} on $X$.
\item[{\rm (iii)}]
A {\sl Radon measure} on $X$ is a Borel measure $\mu$ on $X$ such that
$\mu(K)<\infty$ for each compact set $K\subseteq X$.
\end{enumerate}
\end{definition}
\end{snugshade}

\begin{snugshade}
\begin{theorem}\label{exist-Lebesgue-measure}
There exists a unique Borel measure $\mu$ on $\mathbb{R}$ such that
\begin{equation}\label{muab1}
\mu\big((a,b]\big)=b-a
\end{equation}
for all $a,b\in\mathbb{R}$, with $a<b$.
\end{theorem}
\end{snugshade}

\begin{snugshade}
\begin{definition}\label{def-Lebesgue-measure}
The {\sl Lebesgue measure} on $\mathbb{R}$ is the measure $\mu$
in Theorem \ref{exist-Lebesgue-measure}
\end{definition}
\end{snugshade}



%$\mathfrak{E}\quad \mathfrak{D}\quad \mathfrak{K}\quad \mathfrak{L}\quad \mathfrak{M}\quad \mathfrak{N}\quad
%\mathfrak{P}\quad \mathfrak{Q}\quad \mathfrak{R} \quad \mathfrak{S}\quad \mathfrak{T}\quad \mathfrak{U}\mathfrak{V}\quad \mathfrak{X}\quad \mathfrak{Y}\quad \mathfrak{Z}$


\section{The Lebesgue-Stieltjes integral}
%ver Kolmogorov


\begin{snugshade}
\begin{theorem}\label{teo-image-measure}
Let $(X,\mathcal{A})$ and $(Y,\mathcal{B})$ be two measurable spaces
and let $\mu$ be a measure on $\mathcal{A}$.
Let $F:X\to Y$ be a measurable function.
Define %, for each measurable set $B\in\mathcal{B}$,
%The {\sl image measure} induced by $F$ on $\mathcal{B}$, denoted by $\nu\equiv\mu\circ F^{-1}$,
%is defined by
\begin{equation}\label{imF1}
\nu(B):=\mu\big(F^{-1}(B)\big)\;,\quad B\in\mathcal{B}\;.
\end{equation}
%for each measurable set $B\in\mathcal{B}$.
Then $\nu$ is a measure on $\mathcal{B}$.
\end{theorem}
\end{snugshade}

%\begin{snugshade}
%\begin{definition}\label{def-image-measure}
%Let $(X,\mathcal{A})$ and $(Y,\mathcal{B})$ be two measurable spaces
%and let $\mu$ be a measure on $\mathcal{A}$.
%Let $F:X\to Y$ be a measurable function. The
%{\sl image measure} induced by $F$ on $\mathcal{B}$, denoted by $\nu\equiv\mu\circ F^{-1}$,
%is defined by
%\begin{equation}\label{imF1}
%\nu(B):=\mu\big(F^{-1}(B)\big)
%\end{equation}
%for each measurable set $B\in\mathcal{B}$.
%\end{definition}
%\end{snugshade}

\begin{snugshade}
\begin{definition}\label{def-image-measure}
The measure $\nu$ in Theorem \ref{teo-image-measure}, often denoted by $\mu F^{-1}$,
is called the {\sl image measure} induced by $F$ on $\mathcal{B}$.
\end{definition}
\end{snugshade}

The notion of image measure allows us to introduce new measures from Lebesgue measure,
e.g., the Lebesgue-Stieltjes measure. We begin with the following

\begin{snugshade}
\begin{lemma}\label{lemma-LS1}
Let $F:\mathbb{R}\to\mathbb{R}$ be nonconstant, right-continuous, nondecreasing.
Set $F(\pm\infty):=\lim_{x\to\pm\infty}F(x)$ and $I:=\big(F(-\infty),F(+\infty)\big)$.
Define $f:I\to\mathbb{R}$ by
$$
f(x):=\inf\big\{y\in\mathbb{R}\,:\,x\leq F(y)\big\}\;,\quad x\in I\;.
$$
Then, $F$ is left-continuous and nondecreasing.
Moreover, for each $x\in I$ and $y\in\mathbb{R}$,
$$
f(x)\leq y\quad\mbox{\rm iff}\quad x\leq F(y)\;.
$$
\end{lemma}
\end{snugshade}

\begin{snugshade}
\begin{theorem}\label{Thm-LS1}
Let $F:\mathbb{R}\to\mathbb{R}$ be nonconstant, right-continuous, nondecreasing.
Then there exists a unique Radon measure $\mu_F$ on $\mathbb{R}$ such that
\begin{equation}\label{muabLS1}
\mu_F\big((a,b]\big)=F(b)-F(a)
\end{equation}
for all $a,b\in\mathbb{R}$, with $a<b$.
\end{theorem}
\end{snugshade}

\begin{snugshade}
\begin{definition}\label{def-LS1}
The measure $\mu_F$ in Theorem \ref{Thm-LS1}
is called the {\sl Lebesgue--Stieltjes measure} on $\mathbb{R}$ generated by the function $F$.
\end{definition}
\end{snugshade}

\begin{remark}\em
If $F(x):=x$, then the Lebesgue--Stieltjes measure generated by $F$ coincides with the Lebesgue measure.
\end{remark}

\begin{snugshade}
\begin{definition}\label{def-LSint}
Let $\mu_F$ be the Lebesgue--Stieltjes measure on $\mathbb{R}$ %in the interval $(a,b]$
generated by $F$, and let $a,b\in\mathbb{R}$, with $a<b$.
Let $f:\mathbb{R}\to\mathbb{R}$ be such that $f\cdot\chi_{(a,b]}$ is $\mu_F-$integrable.
The {\sl Lebesgue--Stieltjes integral} of $f$ (with respect to $F$) between $a$ and $b$ is defined by
\begin{equation}\label{LSinteg1}
\int_a^bf\,{\rm d}F:=\int_{(a,b]}f\,{\rm d}\mu_F=\int_{\mathbb{R}}f\cdot \chi_{(a,b]}\,{\rm d}\mu_F\;.
\end{equation}
\end{definition}
\end{snugshade}

\begin{remark}\em
Henceforth, the Lebesgue--Stieltjes integral of a function $f$ with respect to a given function $F$ is simply
the Lebesgue integral of $f$ with respect to the Lebesgue--Stieltjes measure $\mu_F$ generated by $F$.
\end{remark}


\section{Topics on measure and integration}



\section{The Riemann-Stieltjes integral}






\section{Lebesgue-Stieltjes integral \emph{versus} Riemann-Stieltjes integral}


\medskip

\section*{Bibliography}
\medskip

{\small
\begin{enumerate}[label=\emph{\rm [\arabic*]},leftmargin=*]
\item\label{KolmogorovFumini1968-A2} A. Kolmogorov and S. Fomini, {\sl Introductory Real Analysis}, Dover Publications, Inc. (1975).
%\item\label{Lax2002-A2} Peter D. Lax, {\sl Functional Analysis}, John Wiley $\&$ Sons (2002).
\item\label{Norris} J. Norris, {\sl Probability and Measure}
(\text{\scriptsize http://www.statslab.cam.ac.uk/{\textasciitilde{}}james/Lectures/pmall.pdf}).
%({http://www.statslab.cam.ac.uk/~james/Lectures/pmall.pdf}).
%\item\label{ReedSimon1972-A2} M. Reed and B. Simon, {\sl Methods of Modern Mathematical Physics I: Functional Analysis},
%Academic Press (1972).
%\item\label{Rudin1986-A2} W. Rudin, {\sl Real and Complex Analysis}, McGraw-Hill (1986) [paperback edition: 2004].
\end{enumerate}
}



\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\section{No\c c\~oes de tribo e de espa\c co mensur\'avel}
%
%%\hspace{1em}
%
%\begin{definition}
%Seja $X$ um conjunto n\~ao vazio e ${\cal M}\subset {\cal P}(X)$.
%${\cal M}$ diz-se uma $\sigma-${\sf \'algebra}
%(de Boole de conjuntos ou uma {\sf tribo}) sobre $X$ se
%$$
%\begin{array}{cl}
%{\rm (i)} & {\cal M}\not= \phi \\
%\rule{0pt}{1.2em}
%{\rm (ii)} & A,B\in {\cal M} \Rightarrow A^c \in {\cal M} \\
%\rule{0pt}{1.7em}
%{\rm (iii)} & \mbox{\rm $I$ finito ou numer\'avel,
%$A_i\in {\cal M}$ ($i\in I$) \ $\Rightarrow$ \
%$\bigcup_{i\in I}A_i\in {\cal M}$.}
%\end{array}
%$$
%\end{definition}
%
%Obviamente, ${\cal P}(X)$ \'e um primeiro exemplo de tribo.
%Como consequ\^encia imediata da defini\c c\~ao,
%\'e f\'acil de verificar que sendo
%${\cal M}$ uma $\sigma-$\'algebra sobre $X$ e $A,B\in {\cal M}$,
%ent\~ao
%$$
%\begin{array}{cl}
%{\rm (a)} & \phi , X \in {\cal M} \\
%\rule{0pt}{1.2em}
%{\rm (b)} & A \cap B \in {\cal M}  \\
%\rule{0pt}{1.2em}
%{\rm (c)} & A\backslash B\in {\cal M} \, .
%\end{array}
%$$
%%Com efeito,...
%Constata-se sem dificuldade que a propriedade (b) \'e v\'alida
%para intersec\c c\~oes em infinidade numer\'avel, i.e.,
%$$
%\mbox{\rm (b$^{\, \prime}$)} \quad
%\mbox{\rm $I$ finito ou numer\'avel,
%$A_i\in {\cal M}$ ($i\in I$) \ $\Rightarrow$ \
%$\bigcap_{i\in I}A_i\in {\cal M}$.}
%$$
%Assim, podemos concluir que uma $\sigma-$\'algebra de Boole
%\'e est\'avel para as tr\^es opera\c c\~oes fundamentais das
%\'algebras de conjuntos, i.e., a
%complementa\c c\~ao, a reuni\~ao e a interse\c c\~ao, estas
%duas \'ultimas em infinidade numer\'avel
% (o que \'e uma propriedade caracter\'\i stica
%das $\sigma-$\'algebras de Boole).
%
%As $\sigma-$\'algebras de Boole que nos v\~ao interessar s\~ao
%as chamadas $\sigma$-\'algebras de Borel.
%
%\begin{definition}
%Sendo $(X,\tau)$ um espa\c co topol\'ogico (e.t.), a sua
%$\sigma-${\sf \'algebra de Borel} \'e a menor (no sentido da inclus\~ao)
%$\sigma-$\'algebra sobre $X$ que cont\'em $\tau$, dita a
%$\sigma-${\sf \'algebra gerada por} $\tau$.
%Os seus elementos s\~ao chamados os {\sf borelianos} de $X$.
%\end{definition}
%
%Constata-se facilmente que {\it a intersec\c c\~ao de qualquer
%fam\'\i lia de $\sigma-$\'algebras \'e ainda uma $\sigma-$\'algebra},
%pelo que, sendo $(X,\tau)$ um e.t.,
%podemos afirmar que {\it a $\sigma-$\'algebra de Borel gerada por $\tau$
%\'e a intersec\c c\~ao de todas as $\sigma-$\'algebras sobre $X$ que
%cont\^em $\tau$}.
%
%\begin{proposition}
%Seja $X$ um subconjunto de $\bkR^n$ (com a topologia usual) e
%designe ${\cal B}$ a $\sigma-$\'algebra de Borel de $X$. Ent\~ao,
%$$
%\begin{array}{cl}
%{\rm (i)} & \mbox{${\cal B}$ \'e a $\sigma-$\'algebra gerada pelos
%fechados de $X$; } \\
%\rule{0pt}{1.2em}
%{\rm (ii)} & \mbox{${\cal B}$ \'e a $\sigma-$\'algebra gerada pelos
%compactos de $X$. }
%\end{array}
%$$
%\end{proposition}
%
%\noindent{\bf Observa\c c\~ao:}
%
%Decorre da pr\'opria defini\c c\~ao que a $\sigma-$\'algebra de Borel
%sobre um e.t. $X$ \'e a $\sigma-$\'algebra gerada pelos
%conjuntos abertos de $X$.
%Al\'em disso, com uma demonstra\c c\~ao an\'aloga \`a de (i) da
%proposi\c c\~ao precedente, reconhece-se facilmente que esta
%$\sigma-$\'algebra \'e tamb\'em gerada pelos conjuntos fechados de $X$.
%Mais geralmente ainda,
%se $X$ \'e um e.t. de Hausdorff localmente compacto (cada ponto tem
%uma vizinhan\c ca compacta) e $\sigma-$compacto (reuni\~ao
%numer\'avel de compactos), a sua $\sigma-$\'algebra de Borel
%\'e tamb\'em a $\sigma-$\'algebra gerada pelos conjuntos compactos de $X$.
%
%\begin{definition}
%Se ${\cal M}\subset{\cal P}(X)$ \'e uma
%$\sigma-$\'algebra sobre $X$, ao par $(X,{\cal M})$ chamamos
%{\sf espa\c co mensur\'avel}.
%Os subconjuntos de $X$ que sejam elementos de ${\cal M}$
%s\~ao ditos os {\sf subconjuntos mensur\'aveis} de $X$.
%\end{definition}
%
%
%\section{Fun\c c\~oes mensur\'aveis}
%
%\hspace{1em}
%Como se sabe, dados dois e.t.'s $(X,\tau)$ e $(Y,\sigma)$,
%uma aplica\c c\~ao $f:X\rightarrow Y$ diz-se cont\'\i nua se
%$$
%f^{-1}(\sigma)\subset \tau \, .
%$$
%Vamos introduzir nos espa\c cos mensur\'aveis uma no\c c\~ao
%``paralela'' \`a de fun\c c\~ao cont\'\i nua
%nos espa\c cos topol\'ogicos: a de {\it fun\c c\~ao mensur\'avel}.
%
%\begin{definition}
%Sejam $(X,{\cal M})$ e $(Y,{\cal B})$ dois espa\c cos mensur\'aveis.
%Uma aplica\c c\~ao $f:X\rightarrow Y$ diz-se {\sf mensur\'avel} se
%$$
%f^{-1}({\cal B})\subset {\cal M} \, .
%$$
%\end{definition}
%
%No caso de $Y\equiv (Y,\tau)$
%ser um e.t. e ${\cal B}$ a correspondente tribo
%de Borel, a mensurabilidade de $f$ \'e caracterizada pela
%seguinte propriedade:
%$$
%f^{-1}(G) \in {\cal M} \, , \quad \forall G\in\tau \, .
%$$
%Em particular, com $Y=\bkR$ ou $\bkC$ e $\tau$ a topologia usual
%(em $\bkR$ ou $\bkC$), tem-se: (i) $f:X\rightarrow\bkR$ \'e
%mensur\'avel {\it sse} todos os conjuntos da forma
%$f^{-1}(\, ]-\infty,t[\, )$, $t\in\bkR$, s\~ao mensur\'aveis em $X$;
%(ii) $f:X\rightarrow\bkC$ \'e
%mensur\'avel {\it sse} para todo o aberto $U$ em $\bkC$ o conjunto
%$f^{-1}(U)$ \'e mensur\'avel em $X$ ou, equivalentemente,
%{\it sse} as partes real e
%imagin\'aria de $f$ (aplica\c c\~oes de $X$ em $\bkR$)
% s\~ao mensur\'aveis.
%
%\begin{proposition}
%Sejam $(X,\tau)$ e $(Y,\sigma)$ dois e.t.'s e
%$f:X \rightarrow Y$ uma aplica\c c\~ao cont\'\i nua.
%Ent\~ao $f$ \'e mensur\'avel \`a Borel (i.e., relativamente
%\`as tribos de Borel em $X$ e $Y$).
%\end{proposition}
%
%\begin{proposition}
% {\rm (composi\c c\~ao de fun\c c\~oes mensur\'aveis)}
%Se $(X_ 1,{\cal B}_1)$, $(X_2,{\cal B}_2)$ e $(X_3,{\cal B}_3)$
% s\~ao espa\c cos mensur\'aveis e
%$f:X_1 \rightarrow X_ 2$ e  $g:X_2 \rightarrow X_ 3$
%s\~ao fun\c c\~oes mensur\'aveis, ent\~ao tamb\'em
%a composi\c c\~ao $g \circ f:X_1 \rightarrow X_3$ \'e uma
%fun\c c\~ao mensur\'avel.
%\end{proposition}
%
%Em consequ\^encia, se $f$ e $g$ s\~ao duas fun\c c\~oes mensur\'aveis
%reais ou complexas definidas sobre o mesmo espa\c co mensur\'avel
% $(X,{\cal B})$ e $\alpha$ \'e um n\'umero real ou complexo, tamb\'em
%$$
%f+g \, , \quad
%f\cdot g \, , \quad
%\alpha f \, , \quad
%\inf\{f,g\} \, , \quad
%\sup\{f,g\} \, , \quad
%|f| \, , \quad
%\overline{f}
%$$
%($\overline{f}$ representa o conjugado de $f$)
%s\~ao fun\c c\~oes mensur\'aveis.
%Note-se que pode $|f|$ ser mensur\'avel sem que $f$ o seja
%(\'e o que sucede, e.g., com $f:=\chi_A-\chi_{A^c}$
%desde que $A$ n\~ao seja mensur\'avel).
%
%Por outro lado, pode ainda provar-se que
%{\it o limite (pontual) de uma sucess\~ao
%de fun\c c\~oes mensur\'aveis reais ou complexas
%com dom\'\i nio num espa\c co mensur\'avel $X$
%define uma fun\c c\~ao mensur\'avel em $X$}.
%
%\begin{definition}
%Uma fun\c c\~ao  mensur\'avel \'e dita  fun\c c\~ao {\sf simples}
%(ou {\sf em escada}, ou {\sf escalonada}) se o seu contradom\'\i nio
%\'e finito.
%\end{definition}
%
%\begin{proposition}
%Sejam $(X,\tau)$ e $(Y,\sigma)$ dois e.t.'s e suponha-se que
%$(Y,\sigma)$ \'e espa\c co de Hausdorff. Se
%$f:X \rightarrow Y$ \'e uma fun\c c\~ao mensur\'avel e simples,
%digamos, $f(x)=f_i$ se $x\in E_i$, com
%$f(X)=\{ f_1,f_2,\ldots,f_m \}$ e $X=E_1\cup E_2\cup \ldots \cup E_m$,
%ent\~ao cada $E_i$ $(i=1,2,\ldots,m)$ \'e mensur\'avel.
%\end{proposition}
%
%Recorde-se que dado um subconjunto $A$ de um conjunto $X$, chama-se
%{\sf fun\c c\~ao caracter\'\i stica ({\rm ou} indicatr\'\i z) de} $A$,
% e representa-se por $\chi_A$, \`a aplica\c c\~ao de
%$X$ em $\{0,1\}$ definida por
%$$
%\chi_A(x):=\left\{
%\begin{array}{ccl}
%1 & , & x\in A \\
%\rule{0pt}{1.2em}
%0 & , & x\notin A \, .
%\end{array}
%\right.
%$$
%
%\begin{corollary}
%Sendo $(X,{\cal B})$ um espa\c co
%mensur\'avel, um subconjunto $A\subset X$ \'e mensur\'avel
%{\it sse} $\chi_A$ \'e mensur\'avel.
%\end{corollary}
%
%Al\'em disso, uma fun\c c\~ao definida em $X$
% \'e simples {\it sse} se pode  exprimir como uma combina\c c\~ao
%linear finita de fun\c c\~oes caracter\'\i sticas de subconjuntos
%mensur\'aveis de $X$.
%
%De entre as v\'arias representa\c c\~oes poss\'\i veis de
%uma fun\c c\~ao simples $f$ como combina\c c\~ao linear
%de fun\c c\~oes caracter\'\i sticas de subconjuntos mensur\'aveis
%de $X$ {\it h\'a apenas uma}, dita a {\sf forma can\'onica} de $f$,
%$$
%f=\sum_{j=1}^m\alpha_j \chi_{E_j}
%$$
%(para certo $m\in\bkN$), na qual os conjuntos (mensur\'aveis) $E_j$
%s\~ao disjuntos e n\~ao vazios e os coeficientes $\alpha_j$ s\~ao
%distintos dois a dois e todos n\~ao nulos (exclui-se apenas o
%caso $f\equiv 0$ nesta representa\c c\~ao).
%Em particular, $E_j=f^{-1}(\{ \alpha_j\})$ para $j=1,\ldots,m$
%e $\{\alpha_1,\ldots,\alpha_m\}$ \'e o conjunto dos
%valores n\~ao nulos assumidos por $f$.
%
%A proposi\c c\~ao seguinte \'e fundamental
%na teoria do integral de Lebesgue.
%
%\begin{theorem}
%Sejam $X$ um espa\c co mensur\'avel e $f:X \rightarrow \bkR$
%uma aplica\c c\~ao.
%\vspace{0.5em}
%
%{\rm (i)} Se $f$ \'e mensur\'avel
%(relativamente \`a tribo de Borel em $\bkR$) e n\~ao negativa em $X$
%ent\~ao \'e limite pontual de uma sucess\~ao crescente de
%fun\c c\~oes  simples e n\~ao negativas definidas em $X$.
%\vspace{0.5em}
%
%{\rm (ii)} Se $f$ \'e mensur\'avel
%ent\~ao \'e limite pontual de uma sucess\~ao de
%fun\c c\~oes reais simples definidas em $X$.
%\end{theorem}
%
%
%%\section{No\c c\~ao de medida. Propriedades fundamentais. \newline
%%Medidas de Borel e de Lebesgue em $\bkR^n$ }
%
%\section{No\c c\~ao de medida. Propriedades fundamentais. \\
% Medidas de Borel e de Lebesgue em $\bkR^n$ }
%
%\hspace{1em}
%Adiante teremos necessidade de considerar fun\c c\~oes
%com valores em
%$$
%\overline{\bkR}:=\bkR \cup \{-\infty,+\infty\}=[-\infty,+\infty] \, ,
%$$
%a chamada {\sf recta acabada}, relativamente \`a qual se consideram
%as seguintes defini\c c\~oes:
%\vspace{0.5em}
%
%\hspace{2em} (i) \ $-\infty < +\infty$ ;
%
%\hspace{2em} (ii) \ $-\infty < t< +\infty \, , \quad \forall t \in\bkR$ ;
%
%\hspace{2em} (iii) \ $t+(\pm\infty)= (\pm\infty)+t=\pm\infty
%                    \, , \quad \forall t \in\bkR$ ;
%
%\hspace{2em} (iv) \ $(\pm\infty)+(\pm\infty)=\pm\infty$ ;
%
%\hspace{2em} (v) \ $t \cdot (\pm\infty)=
%(\pm\infty) \cdot t=\left\{
%\begin{array}{ccl}
%\pm\infty & {\rm se} & t>0 \\
%%\rule{0pt}{1.2em}
%0 & {\rm se} & t=0 \\
%%\rule{0pt}{1.2em}
%\mp\infty & {\rm se} & t<0
%\end{array}
%\right. \, , \quad \forall t \in\overline{\bkR}$ .
%\vspace{0.5em}
%
%N\~ao se define
%$(\pm\infty)+(\mp\infty)$ nem $(\pm\infty)-(\mp\infty)$.
%
%\'E poss\'\i vel introduzir uma topologia em $\overline{\bkR}$
%relativamente \`a qual $\bkR$ \'e um aberto denso em
% $\overline{\bkR}$ (o que explica a nota\c c\~ao  $\overline{\bkR}$
%para a recta acabada).
%Nesta topologia, uma parte $A$ de $\overline{\bkR}$ \'e um
%aberto se e s\'o se
%(i) para todo o $x\in A\cap \bkR$ existe um intervalo aberto
%de centro em $x$ e contido em $A$;
%(ii) quando $+\infty$ (resp. $-\infty$) pertence a $A$
%existe um intervalo $]a,+\infty]$ com $a\in\bkR$
%(resp.  $[-\infty,b[$ com $b\in\bkR$) contido em $A$.
%\'E relativamente a essa topologia
%em  $\overline{\bkR}$ que se pode afirmar que uma aplica\c c\~ao
%$f:X\rightarrow \overline{\bkR}$ (onde $X$ \'e um espa\c co
%mensur\'avel) \'e mensur\'avel em $X$ {\it sse} os conjuntos
%$$
%f^{-1}(\, ]-\infty,t[\, ) \, , \quad -\infty<t\leq +\infty \, ,
%$$
%s\~ao mensur\'aveis.
%
%\begin{definition}
%Seja $(X,{\cal M})$ um espa\c co mensur\'avel.
%Chama-se {\sf medida} (positiva) em $X$ a toda a aplica\c c\~ao
%$$
%\mu : {\cal M} \rightarrow \overline{\bkR}_0^+:=[0,+\infty ]
%$$
%tal que
%\vspace{0.5em}
%
%\hspace{2em} {\rm (i)} $\quad \mu(\phi)=0$
%\vspace{0.5em}
%
%\hspace{2em} {\rm (ii)} $\quad \mu$ \'e $\sigma-${\sf aditiva}, i.e.,
%se $I$ \'e um conjunto de \'\i ndices finito ou numer\'avel,
%$A_i\in {\cal M}$ ($i\in I$) e $A_i\cap A_j=\phi$ ($i\not= j$), ent\~ao
%$$
%\mu\left( \bigcup_{i\in I}A_i \right) = \sum_{i\in I}\mu(A_i)\, .
%$$
%\end{definition}
%
%\noindent{\bf Observa\c c\~oes:}
%\vspace{0.5em}
%
%1. $\mu(E)$ diz-se a {\sf medida do conjunto} $E\in {\cal M}$.
%\vspace{0.5em}
%
%2. O terno ordenado $(X,{\cal M},\mu)$ diz-se um {\sf espa\c co de
%medida} ou {\sf espa\c co mensurado} e, quando n\~ao houver ambiguidade
%no contexto, ser\'a representado apenas por $X$.
%\vspace{0.5em}
%
%3. Se $\mu(X)<+\infty$, diz-se que $\mu$ \'e uma medida
%{\sf finita}. Se $X$ se puder escrever como uma reuni\~ao
%numer\'avel de subconjuntos mensur\'aveis de $X$ com medida finita,
%diz-se que $\mu$ \'e $\sigma$-{\sf finita}.
%
%\begin{proposition}
%Seja $(X,{\cal M},\mu)$ um espa\c co mensurado.
%\vspace{0.5em}
%
%{\rm (i)} Se $A,B\in {\cal M}$ e $A\subset B$
%ent\~ao $\mu(A)\leq \mu(B)$.
%\vspace{0.5em}
%
%{\rm (ii)} Se $A,B\in {\cal M}$ e $A\subset B$ e $\mu(A)<+\infty$
%ent\~ao
%$$
%\mu(B\backslash A)= \mu(B)-\mu(A) \, .
%$$
%
%{\rm (iii)} Se $A=\bigcup_{n=1}^{\infty}A_n$, onde
%$A_n\in {\cal M}$ e $A_n\subset A_{n+1}$ para todo o $n\in\bkN$,
%ent\~ao
%$$
%\lim_{n\rightarrow+\infty}\mu(A_n)=\mu(A) \, .
%$$
%
%{\rm (iv)} Se $A=\bigcap_{n=1}^{\infty}A_n$,
%$A_n\in {\cal M}$ e $A_{n+1}\subset A_{n}$ para $n\in\bkN$
%e $\mu(A_1)<\infty$,
%ent\~ao
%$$
%\lim_{n\rightarrow+\infty}\mu(A_n)=\mu(A) \, .
%$$
%\end{proposition}
%
%Em seguida vamos referir alguns aspectos importantes e \'uteis
%na constru\c c\~ao de medidas. Como anteriormente observ\'amos,
%dado um conjunto $X\not=\phi$, uma $\sigma-$\'algebra sobre $X$
%pode caracterizar-se do seguinte modo: \'e toda a fam\'\i lia
%de elementos de ${\cal P}(X)$ est\'avel para as
%tr\^es opera\c c\~oes elementares --
%a complementa\c c\~ao, a reuni\~ao
%e a intersec\c c\~ao, estas \'ultimas em infinidade numer\'avel.
%No caso de se exigir a estabilidade destas duas opera\c c\~oes
%apenas em n\'umero finito, a fam\'\i lia diz-se uma
%{\sf \'algebra de Boole} sobre $X$ (note-se que esta
%caracteriza\c c\~ao encerra em si condi\c c\~oes
%super-abundantes, mas
%\'e \'util apresent\'a-la como defini\c c\~ao!). Claro que toda
%a $\sigma-$\'algebra \'e uma \'algebra (porque se a classe \'e
%est\'avel para as tr\^es opera\c c\~oes elementares em infinidade
%numer\'avel, naturalmente que tamb\'em o \'e em n\'umero finito).
%
%Vamos agora explicar como \'e que a possibilidade de definir
%uma medida sobre uma \'algebra permite obter uma medida sobre
%a tribo gerada por essa \'algebra (i.e., a menor tribo que
%cont\'em a \'algebra). Para isso, come\c camos por
%generalizar o conceito de medida, definindo medida sobre uma
%parte de ${\cal P}(X)$ que n\~ao seja necessariamente uma
%tribo.
%
%\begin{definition}
%Seja $X$ um conjunto n\~ao vazio e ${\cal A}\subset {\cal P}(X)$.
%Uma aplica\c c\~ao
%$$
%\mu : {\cal A} \rightarrow \overline{\bkR}_0^+:=[0,+\infty ]
%$$
%diz-se uma {\sf medida (em $X$) sobre} ${\cal A}$ se
%\vspace{0.5em}
%
%\hspace{2em} {\rm (i)} $\quad \mu(\phi)=0$
%\vspace{0.5em}
%
%\hspace{2em} {\rm (ii)} $\quad \mu$ \'e {\sf aditiva}, i.e., se
%$ A,B\in {\cal A}$ e $A\cap B=\phi$ ent\~ao
%$\ \mu(A\cup B)=\mu(A)+\mu(B)$
%\vspace{0.5em}
%
%\hspace{2em} {\rm (iii)} \
% se $A=\bigcup_{n=1}^{\infty}A_n\i {\cal A}$, onde
%$A_n\in {\cal M}$ e $A_n\subset A_{n+1}$ para todo o $n\in\bkN$,
%ent\~ao
%$$
%\lim_{n\rightarrow+\infty}\mu(A_n)=\mu(A) \, .
%$$
%\end{definition}
%
%No caso de ${\cal A}$ ser uma tribo, esta defini\c c\~ao
%\'e equivalente \`a defini\c c\~ao de
%medida anteriormente formulada (sobre uma tribo).
%
%De acordo com a defini\c c\~ao precedente, podemos falar em
%medida definida sobre uma \'algebra de partes de um conjunto
%$X\not=\phi$. Tem ent\~ao lugar o important\'\i ssimo
%
%\begin{theorem}
%{\rm {\bf (do prolongamento da medida)}}  \
%Dada uma medida $\lambda$ sobre uma \'algebra
%${\cal A}\subset {\cal P}(X)$, existe uma medida $\mu$
%sobre a tribo ${\cal M}$ gerada por ${\cal A}$ cuja restri\c c\~ao
%a ${\cal A}$  coincide com $\lambda$.
%Al\'em disso, se $\lambda$ for finita ou $\sigma-$finita,
%ent\~ao o prolongamento $\mu$ de $\lambda$ \'e \'unico.
%\end{theorem}
%
%Na prova deste resultado (que aqui n\~ao tem lugar), \'e
%utilisado o crit\'erio seguinte, que \'e tamb\'em
%\'util noutras situ\c c\~oes.
%
%\begin{theorem}
%{\rm {\bf (crit\'erio da igualdade das medidas)}} \
%Duas medidas definidas num espa\c co mensur\'avel $(X,{\cal M})$
%s\~ao coincidentes sempre que coincidam sobre uma \'algebra
%geradora da tribo ${\cal M}$ e nela sejam finitas ou
%$\sigma-$finitas.
%\end{theorem}
%
%O Teorema do prolongamento de uma medida assegura a
%exist\^encia (e unicidade, sob certas restri\c c\~oes --
%que nos casos que nos v\~ao interessar s\~ao sempre verificadas)
%de uma medida sobre uma tribo sempre que se conhe\c ca a
%sua restri\c c\~ao a uma \'algebra.
%\'E, por isso, \'util dispor de crit\'erios que permitam
% determinar a \'algebra a partir de classes mais restritas
%(i.e., determinar a \'algebra a partir de uma classe
%geradora dessa \'algebra). Com o prop\'osito de estabelecer
%tais crit\'erios, vamos introduzir a defini\c c\~ao
%de semi-\'algebra.
%
%\begin{definition}
%Seja $X$ um conjunto n\~ao vazio e ${\cal S}\subset {\cal P}(X)$.
%${\cal S}$ diz-se uma {\sf semi-\'algebra}
%(de Boole) sobre $X$ se
%$$
%\begin{array}{cl}
%{\rm (i)} & \phi, X \in {\cal S}  \\
%\rule{0pt}{1.2em}
%{\rm (ii)} & A,B\in {\cal S} \Rightarrow A\cap B \in {\cal S} \\
%\rule{0pt}{1.3em}
%{\rm (iii)} & A \in {\cal S} \ \Rightarrow \quad
%\exists_{m\in\bkN} \, \exists_{A_1,\ldots A_m\in {\cal S}} \, : \,
%A^c=\bigcup_{i=1}^m A_i \, .
%\end{array}
%$$
%\end{definition}
%
%Por exemplo, a classe de todos os intervalos de $\bkR$
%(abertos, semi-abertos ou fechados, de comprimento finito ou infinito)
%forma uma semi-\'algebra sobre $\bkR$.
%
%A proposi\c c\~ao seguinte mostra como gerar a \'algebra
%a partir de uma semi-\'algebra geradora.
%
%\begin{theorem}
%{\rm {\bf (da gera\c c\~ao da \'algebra)}} \
%Se $\, {\cal S}$ \'e uma semi-\'algebra de Boole sobre $X$, a
%\'algebra de Boole sobre $X$ gerada por ${\cal S}$
%(i.e., a menor \'algebra de Boole que cont\'em ${\cal S}$) \'e
%constitu\'\i da pelas reuni\~oes finitas dos subconjuntos de
%${\cal S}$ disjuntos dois a dois.
%\end{theorem}
%
%Muitos dos conceitos e resultados precedentes tiveram origem
%no processo de resolu\c c\~ao do problema de
%``medir os subconjuntos de $\bkR$'' (ou, mais geralmente,
%de $\bkR^n$), mas, \'e claro, de forma razo\'avel, i.e.,
%de modo que o conceito de medida a introduzir sobre $\bkR$
%tenha propriedades que estejam de acordo com a intui\c c\~ao
%que o problema suscita.
%Os exemplos 2 e 3 a seguir tratam, justamente, do
%problema da medida em $\bkR^n$.
%\vspace{0.5em}
%
%\noindent{\bf Exemplos:}
%\vspace{0.5em}
%
%1-{\sf Medida contagem.}
%Sendo $X$ um conjunto finito ou infinito numer\'avel,
%chama-se {\sf medida contagem} (ou {\sf medida cardinal})
%\`a medida $\mu$ sobre ${\cal P}(X)$ que atribui a cada subconjunto
%de $X$ o seu cardinal (considerando que este \'e $+\infty$ se $X$
%for infinito).
%\vspace{0.5em}
%
%2-{\sf Medida de Borel (ou de Borel-Lebesgue,
%ou medida uniforme) em $\bkR^n$.}
%Comecemos por considerar o caso $n=1$.
%Assim, fixados dois pontos $a$ e $b$ da recta real,
%extremos de um intervalo $I$, aberto, fechado ou semi-aberto,
%\'e natural associar como medida do intervalo $I$ a sua
%amplitude, i.e., definimos a medida do intervalo $I$ por
%$$
%\mu_1(I):=|b-a| \, .
%$$
%\'E f\'acil de verificar que o conjunto dos intervalos de $\bkR$
%\'e uma semi-\'algebra que
%(pelo Teorema da gera\c c\~ao da \'algebra)
%gera uma \'algebra cujos elementos s\~ao as reuni\~oes
%finitas dos subconjuntos disjuntos da semi-\'algebra.
%Portanto, cada subconjunto $A$ desta \'algebra \'e da forma
%$$
%A=\cup_{j=1}^mI_j
%$$
%onde $I_1,\ldots,I_m$ s\~ao intervalos de $\bkR$
%disjuntos dois a dois.
%Assim, designando por $a_j$ e $b_j$ os extremos
%de $I_j$, como $\mu_1(I_j)=|b_j-a_j|$, para preservar a aditividade
%devemos definir
%$$
%\mu_1(A):=\sum_{i=1}^m |b_j-a_j| \, ,
%$$
%e fica assim definida a medida sobre a \'algebra.
%Pelo Teorema do prolongamento da medida podemos prolongar
%esta medida (sobre a \'algebra)
% \`a tribo gerada pela \'algebra, a qual coincide
%com a tribo de Borel de $\bkR$ (como facilmente se reconhece,
%observando que a tribo de Borel \'e tamb\'em gerada pelo
%conjunto de todos os intervalos de $\bkR$, j\'a que qualquer
%intervalo \'e um boreliano em $\bkR$,
%i.e., pertence \`a tribo de Borel sobre $\bkR$).
%A medida definida por este prolongamento n\~ao \'e finita,
%pois $\mu_1(\bkR)=\mu_1(\, ]-\infty,+\infty[\, )=+\infty$;
%por\'em, \'e $\sigma-$finita, porque podemos escrever
%$\bkR=\cup_{n\in\bkZ} \, [n,n+1]$ com
%$\mu_1([n,n+1])=1<+\infty$.
%Conclui-se (novamente pelo Teorema do prolongamento) a
%unicidade desta medida $\mu_1$ sobre a tribo de Borel,
%recebendo a designa\c c\~ao de {\sf medida de Borel} sobre $\bkR$.
%
%Note-se que, em particular,  a medida de Borel de um ponto
%(i.e., de um conjunto singular) \'e nula,
%$\mu_1(\{a\})=0$, bem como a medida de Borel de qualquer
%subconjunto numer\'avel de $\bkR$. Em particular,
%$$
%\mu_1(\bkQ)=0 \, .
%$$
%Referimos, por\'em, que pode haver borelianos ``muito estranhos''
%com medida de Borel nula,
%incluindo com a pot\^encia do cont\'\i nuo -- um exemplo \'e
%fornecido pelo famoso conjunto tri\'adico de Cantor.
%
%No caso geral, por uma costru\c c\~ao an\'aloga
%define-se a {\sf medida de Borel} em $\bkR^n$, que
%\'e a medida $\mu_n$ definida na tribo de Borel de $\bkR^n$
%que verifica
%$$
%\mu_n\left( \prod_{i=1}^n [a_i,b_i] \right)=
%\prod_{i=1}^n (b_i-a_i)
%\, , \quad (a_i,b_i \in\bkR \, , \ a_i\leq b_i) \, ,
%$$
%e o mesmo se obt\'em se se considerarem intervalos abertos
%ou semi-abertos em vez de intervalos fechados.
%\vspace{0.5em}
%
%3-{\sf Medida de Lebesgue em $\bkR^n$.} Para definir esta medida
%\'e necess\'ario introduzir alguns conceitos.
%Uma medida $\mu$ \'e dita {\sf completa} se
%$$
%\mu(A)=0 \  , \  B\subset A \quad \Rightarrow \quad
%\mbox{$B$ mensur\'avel} \ {\rm e} \ \mu(B)=0 \, .
%$$
%Prova-se que {\it toda a medida $\mu$ sobre uma tribo ${\cal M}$
%se pode extender a uma medida completa $\overline{\mu}$,
%dita o {\sf completamento de} $\mu$, definida sobre uma
%classe mais ampla}. Vejamos, sumariamente, como \'e definida
%esta extens\~ao. Seja
%$$
%\overline{{\cal M}}:=
%\{ \, S\Delta N \, | \, S\in {\cal M}
%\mbox{ e $\exists_{A\in {\cal M}} \, : \, N\subset A$ e }
%\mu(A)=0 \, \} \, ,
%$$
%onde $S\Delta N$ \'e a {\sf diferen\c ca sim\'etrica}
%dos conjuntos $S$ e $N$,
%$$
%S\Delta N := (S\cap N^c)\cup (S^c\cap N) \, .
%$$
%Claramente, ${\cal M} \subset \overline{{\cal M}}$
%(j\'a que
%$S\in {\cal M} \Rightarrow S=S\Delta \phi \in \overline{{\cal M}}$).
%O completamento $\overline{\mu}$ de $\mu$
% \'e a medida definida sobre $\overline{{\cal M}}$ por
%$$
%\overline{\mu}(S\Delta N):=\mu(S) \, .
%$$
%Trata-se obviamente de uma extens\~ao de $\mu$.
%
%Pode mostrar-se que a medida de Borel sobre $\bkR^n$
%(que \'e definida sobre a tribo de Borel de $\bkR^n$)
%n\~ao \'e completa. Este facto motiva a defini\c c\~ao seguinte.
%
%\begin{definition}
%Chama-se {\sf medida de Lebesgue em} $\bkR^n$ ao completamento
%da medida de Borel em $\bkR^n$.
%Designando por ${\cal B}_{\bkR^n}$ a tribo de Borel em $\bkR^n$,
%a correspondente tribo $\overline{{\cal B}_{\bkR^n}}$ diz-se
%{\sf tribo de Lebesgue em} $\bkR^n$.
%\end{definition}
%
%Naturalmente, sendo uma extens\~ao da medida de Borel,
%representando por $\lambda_n$ a medida de Lebesgue
%em $\bkR^n$ tem-se ainda
%$$
%\lambda_n\left( \prod_{i=1}^n [a_i,b_i] \right)=
%\prod_{i=1}^n (b_i - a_i)
%\, , \quad (a_i,b_i \in\bkR \, , \ a_i\leq b_i) \, .
%$$
%
%Prova-se que
%{\it a medida de Lebesgue \'e invariante por transla\c c\~ao},
%i.e., se $x\in\bkR^n$ e $S\subset \bkR^n$ (mensur\'avel), ent\~ao
%$$
%\lambda_n(x+S)=\lambda_n(S) \, ,
%$$
%onde $x+S:=\{ x+s : s\in S \}$.
%
%Finalmente, referimos que existem subconjuntos de $\bkR^n$
%que n\~ao est\~ao na tribo de Lebesgue. Por\'em, a constru\c c\~ao
%de tais conjuntos \'e, em geral, muito artificial
%(os exemplos mais divulgados s\~ao normalmente constru\'\i dos
%recorrendo ao axioma da escolha).
%
%\section{Integral de Lebesgue. Teoremas fundamentais.}
%
%\hspace{1em} Se $f$ \'e uma fun\c c\~ao que toma valores em $\bkR$,
% chama-se
%{\sf parte positiva} de $f$ \`a fun\c c\~ao $f^+$ definida por
%$$
%f^+:=\sup\{ f,0 \} \, ;
%$$
%analogamente, a {\sf parte negativa} de $f$ \'e a
% fun\c c\~ao $f^-$ definida por
%$$
%f^-:=-\inf\{ f,0 \} \, .
%$$
%Constata-se de imediato que
%$$
%f^+ \geq 0 \, , \quad
%f^- \geq 0 \, , \quad
%f=f^+-f^- \, , \quad
%|f|=f^++f^- \, .
%$$
%Al\'em disso,
%se $f$ \'e mensur\'avel, tamb\'em $f^+$ e $f^-$ o s\~ao.
%
%\begin{definition}
% {\rm {\bf (integral de Lebesgue)}}
% Seja $(X,{\cal M},\mu)$ um espa\c co mensurado e
%$f$ uma fun\c c\~ao real ou complexa mensur\'avel em $X$.
%O {\sf integral de $f$ relativamente a} $\mu$,
%$\displaystyle \int_X f{\rm d}\mu$,
%define-se de acordo com as seguintes etapas:
%\vspace{0.5em}
%
%{\rm (i)} \ se $f$ \'e uma fun\c c\~ao simples, digamos,
%$f=\sum_{i=1}^m\alpha_i \chi_{E_i}$, definimos
%$$
%\int_X f \, {\rm d}\mu := \sum_{i=1}^m \alpha_i \mu(E_i) \, ;
%$$
%
%{\rm (ii)} \ se $f$ \'e n\~ao negativa, definimos
%$$
%\int_X f \, {\rm d} \mu :=
% \sup_{\stackrel{\scriptstyle 0\leq \varphi \leq f}{\stackrel{}{
%       \mbox{\scriptsize \rm $\varphi$ simples}}}}
%\int_X \varphi \, {\rm d}\mu  \, ;
%$$
%
%{\rm (iii)} \ $f$ diz-se {\sf integr\'avel
% (ou som\'avel)  \`a Lebesgue em $X$
%relativamente a $\mu$} (ou, simplesmente,
%$\mu-${\sf integr\'avel em} $X$) se
%$$
%\int_X |f| \,{\rm d} \mu <+\infty \, ;
%$$
%
%{\rm (iv)} \ se $f$ \'e real e $\mu-$integr\'avel, definimos
%$$
%\int_X f \, {\rm d} \mu :=
% \int_X f^+ \, {\rm d}\mu -
%\int_X f^- \, {\rm d}\mu \, ;
%$$
%
%{\rm (v)} \ se $f$ \'e complexa e $\mu-$integr\'avel, digamos,
%$f = f_r+if_i$,
%definimos
%$$
%\int_X f \, {\rm d} \mu :=
% \int_X f_r \, {\rm d}\mu +
%i \int_X f_i \, {\rm d}\mu \, .
%$$
%\end{definition}
%
%\noindent{\bf Observa\c c\~oes:}
%\vspace{0.5em}
%
%1. O integral de uma fun\c c\~ao mensur\'avel
% n\~ao negativa existe sempre -- pode \'e ser infinito!.
%Al\'em disso, quando $f\geq0$ em $X$, \'e usual escrever
%$\int_X f \, {\rm d}\mu=+\infty$ para indicar que
%$f$ n\~ao \'e $\mu-$integr\'avel sobre $X$.
%\vspace{0.5em}
%
%2. Resulta imediatamente da defini\c c\~ao que uma fun\c c\~ao
%mensur\'avel $f$ \'e integr\'avel \`a Lebesgue
%se e s\'o se $|f|$ o for. Recorde-se que isto n\~ao sucede no
%caso do integral de Riemann.
%\vspace{0.5em}
%
%3. Quando $\mu=\lambda_n$ \'e a medida de Lebesgue, normalmente escreve-se
%$\displaystyle \int_X f {\rm d}x_1 \ldots {\rm d}x_n$ ou,
%simplesmente, $\displaystyle \int_X f{\rm d}x$,
%em vez de
%$\displaystyle \int_X f{\rm d}\lambda_n$.
%\vspace{0.5em}
%
%4. Como se sabe, na defini\c c\~ao de integral de Riemann
%consideram-se parti\c c\~oes do dom\'\i nio da fun\c c\~ao.
%Por\'em, na defini\c c\~ao do integral de Lebesgue estamos
%sobretudo interessados nos valores que a fun\c c\~ao
%assume, i.e., no contradom\'\i nio da fun\c c\~ao --
%em certo sentido, podemos dizer que no
%integral de Lebesgue se
%consideram parti\c c\~oes do contradom\'\i nio da fun\c c\~ao.
%\vspace{0.5em}
%
%
%\begin{theorem}
%{\rm {\bf (da converg\^encia mon\'otona)}} \
%Seja $(X,{\cal M},\mu)$ um espa\c co mensurado e $\{f_n\}_{n\in\bkN}$
%uma sucess\~ao de fun\c c\~oes mensur\'aveis em $X$ com valores em $\overline{\bkR}$.
%Suponha-se que
%$$
%\begin{array}{cl}
%{\rm (i)} & f_n\geq 0 \quad \mbox{\rm a.e. em $X$}  \\
%\rule{0pt}{1.2em}
%{\rm (ii)} & \{f_n\}_{n\in\bkN} \quad \mbox{\rm \'e mon\'otona crescente a.e.}  \, .
%\end{array}
%$$
%Nestas condi\c c\~oes,
%$$
%\int_X \left( \lim_{n\rightarrow +\infty}f_n \right) \, {\rm d}\mu =
%\lim_{n\rightarrow +\infty} \, \int_{X}f_n \, {\rm d}\mu \, .
%$$
%\end{theorem}
%
%
%\noindent{\bf Observa\c c\~oes:}
%\vspace{0.5em}
%
%1. Note-se que $\displaystyle\lim_{n\rightarrow +\infty}f_n$
%est\'a definido a.e. como uma
%fun\c c\~ao n\~ao negativa com valores em $\overline{\bkR}$
%\vspace{0.3em}
%
%2. Decorre do Teorema que $\displaystyle\lim_{n\rightarrow +\infty}f_n$
%\'e integr\'avel {\it sse}
%a sucess\~ao num\'erica
%$\{ \int_{X}f_n \, {\rm d}\mu \}_{n\in\bkN}$ \'e majorada em $\bkR$.
%\vspace{0.5em}
%
%Como corol\'ario, pode provar-se o seguinte
%\vspace{0.5em}
%
%
%\begin{theorem}
%{\rm {\bf (de Beppo-Levi)}} \
%Seja $(X,{\cal M},\mu)$ um espa\c co mensurado e $\{f_n\}_{n\in\bkN}$
%uma sucess\~ao de fun\c c\~oes n\~ao negativas (a.e.)
% e mensur\'aveis em $X$,
% com valores em $\overline{\bkR}$, e seja $f$ a soma pontual (definida a.e.)
%$$
%f(x)=\sum_{n\in\bkN}f_n(x) \, .
%$$
%Ent\~ao
%$$
%\int_X f \, {\rm d}\mu =
%\sum_{n\in\bkN} \, \int_{X}f_n \, {\rm d}\mu \, .
%$$
%Em particular, $f$ \'e $\mu-$integr\'avel se e s\'o se
%todas as fun\c c\~oes $f_n$ s\~ao $\mu-$integr\'aveis e a
%s\'erie num\'erica
%$\sum_{n\in\bkN} \, \int_{X}f_n \, {\rm d}\mu$
%\'e convergente em $\bkR$.
%\end{theorem}
%\vspace{0.5em}
%
%O resultado central na Teoria do Integral de Lebesgue \'e,
%sem d\'uvida, o seguinte
%
%\begin{theorem}
%{\rm {\bf (da converg\^encia dominada de Lebesgue)}} \
%Seja $(X,{\cal M},\mu)$ um espa\c co mensurado e $\{f_n\}_{n\in\bkN}$
%uma sucess\~ao de fun\c c\~oes complexas e $\mu-$mensur\'aveis em $X$.
%Suponha-se que
%$$
%\begin{array}{cl}
%{\rm (i)} & f_n\rightarrow 0 \quad \mbox{\rm a.e. em $X$}  \\
%\rule{0pt}{1.2em}
%{\rm (ii)} & \mbox{\rm existe uma fun\c c\~ao $g$ que \'e $\mu-$integr\'avel em $X$ e tal que}
%\end{array}
%$$
%$$
%|f_n|\leq g \quad \mbox{\rm a.e. em $X$, \ para todo o $n\in\bkN$} \, .
%$$
%Nestas condi\c c\~oes, $f_n$ e $f$ s\~ao $\mu-$integr\'aveis em $X$ e
%$$
%\int_X f \, {\rm d}\mu =
%\lim_{n\rightarrow +\infty} \, \int_{X}f_n \, {\rm d}\mu \, .
%$$
%\end{theorem}
%
%Como aplica\c c\~ao do teorema da converg\^encia dominada de Lebesgue,
%podemos facilmente estabelecer os seguintes resultados
%relacionados com a continuidade e possibilidade de deriva\c c\~ao
%de um integral param\'etrico do tipo
%$$
%F(t):=\int_X f(x,t)\, {\rm d}\mu(x) \, ,
%$$
%onde $t$ \'e um par\^ametro real.
%
%\begin{corollary}
%{\rm {\bf (passagem do limite sob o sinal de integral)}} \
%Seja $(X,{\cal M},\mu)$ um espa\c co mensurado,
%$I$ um subconjunto de n\'umeros reais,
%$t_0$ um ponto de acumula\c c\~ao de $I$ e
%$$
%f:X\times I \rightarrow \bkC
%$$
%uma fun\c c\~ao tal que para todo o $t\in I$ as fun\c c\~oes
%$
%x \mapsto f(x,t)
%$
%s\~ao $\mu-$mensur\'aveis em $X$ e
%$$
%\lim_{t\rightarrow t_0} f(x,t) = h(x) \quad \mbox{\rm a.e. em $X$}
%$$
%(para uma fun\c c\~ao $h$).
%Suponha-se ainda que existe uma fun\c c\~ao $g$, $\mu-$integr\'avel em $X$,
%tal que
%$$
%|f(x,t)| \leq g(x) \quad \mbox{\rm a.e. em $X$ para todo o $t\in I\, $.}
%$$
%Nestas condi\c c\~oes,
%$$
%\begin{array}{cl}
%{\rm (i)} & \mbox{\rm as fun\c c\~oes $x\mapsto f(x,t)$ s\~ao
%$\mu-$integr\'aveis para todo o $t\in I$} \\
%\rule{0pt}{1.2em}
%{\rm (ii)} & \mbox{\rm $h$ \'e $\mu-$integr\'avel em $X$} \\
%\rule{0pt}{1.8em}
%{\rm (iii)} & \displaystyle{\lim_{t\rightarrow t_0}
%\int_X f(x,t)\, {\rm d}\mu(x)=\int_X h(x)\, {\rm d}\mu(x) \, .}
%\end{array}
%$$
%\end{corollary}
%
%
%\begin{corollary}
%{\rm {\bf (deriva\c c\~ao sob o sinal de integral)}} \
%Seja $(X,{\cal M},\mu)$ um espa\c co mensurado,
%$I$ um intervalo de n\'umeros reais e
%$$
%f:X\times I \rightarrow \bkC
%$$
%uma fun\c c\~ao tal que para todo o $t\in I$ as fun\c c\~oes
%$
%x\mapsto f(x,t)
%$
%s\~ao $\mu-$integr\'aveis em $X$,
%enquanto que para $x$ a.e. em $X$ as fun\c c\~oes $t\mapsto f(x,t)$ s\~ao
%diferenci\'aveis em $I$.
%Suponha-se ainda que existe uma fun\c c\~ao $g$, definida e $\mu-$integr\'avel em $X$,
%tal que
%$$
%\left| \frac{\partial f}{\partial t}(x,t) \right| \leq g(x) \quad \mbox{\rm a.e. em $X$}
%$$
%para todo o $t\in I$.
%
%Designe
%$$
%F(t):=\int_Xf(x,t)\, {\rm d}\mu(x) \, , \quad t\in I \, .
%$$
%Ent\~ao
%$$
%\begin{array}{cl}
%{\rm (i)} & \mbox{\rm $F$ \'e diferenci\'avel em $I$} \\
%\rule{0pt}{1.5em}
%{\rm (ii)} & \mbox{\rm as fun\c c\~oes
%$\displaystyle x\mapsto \frac{\partial f}{\partial t}(x,t)$ s\~ao
%$\mu-$integr\'aveis em $X$ para todo o $t\in I$} \\
%\rule{0pt}{2.0em}
%{\rm (iii)} & \displaystyle{\frac{{\rm d} F}{{\rm d} t}(t) =
%\int_X \frac{\partial f}{\partial t}(x,t) \, {\rm d}\mu(x) \, ,
%\ t\in I \, .}
%\end{array}
%$$
%\end{corollary}
%
%Para concluir esta sec\c c\~ao vamos referir um resultado
%(Teorema de Fubini-Lebesgue) que,
%conjuntamente com o teorema da converg\^encia dominada
%de Lebesgue e a teoria dos espa\c cos $L^p$ (que supomos conhecida
%nos seus tra\c cos gerais), constituem os instrumentos mais \'uteis
%da Teoria do Integral de Lebesgue. Este resultado fundamental
%diz respeito aos integrais m\'ultiplos de Lebesgue.
%Come\c camos com a seguinte
%
%\begin{definition}
%Sejam $(X,{\cal S})$ e $(Y,{\cal T})$
%dois espa\c cos mensur\'aveis.
%\vspace{0.5em}
%
%{\rm (i)} \
%Chama-se {\sf rect\^angulo mensur\'avel} em $X\times Y$ a
%todo o conjunto da forma $E\times F$, onde
%$E\in {\cal S}$ e $F\in {\cal T}$.
%\vspace{0.5em}
%
%{\rm (ii)} \
%Chama-se {\sf tribo produto} em $X\times Y$ \`a tribo gerada
% pelos rect\^angulos mensur\'aveis, e designa-se por
%${\cal S} \times {\cal T}$. O espa\c co $X\times Y$ munido
%com a tribo produto ${\cal S} \times {\cal T}$ designa-se por
%{\sf espa\c co mensur\'avel produto} de
%$(X,{\cal S})$ e $(Y,{\cal T})$.
%\end{definition}
%
%\noindent{\bf Observa\c c\~ao:}
%\vspace{0.5em}
%
%Se $X$ e $Y$ s\~ao espa\c cos topol\'ogicos e
%se ${\cal B}_X$ e ${\cal B}_Y$ designam as tribos de Borel
%em $X$ e $Y$, respectivamente, ent\~ao
%${\cal B}_X \times {\cal B}_Y$ {\it est\'a contida}
% na tribo ${\cal B}_{X\times Y}$ dos borelianos de $X\times Y$
%(e a inclus\~ao pode ser estrita).
%Por\'em  se $X$ e $Y$ s\~ao espa\c cos m\'etricos separ\'aveis
%ent\~ao ${\cal B}_X \times {\cal B}_Y={\cal B}_{X \times Y}$.
%
%\begin{proposition}
%Sejam $(X,{\cal S},\mu)$ e $(Y,{\cal T},\nu)$
%dois espa\c cos mensurados e $f:X\times Y\rightarrow \bkC$
%uma fun\c c\~ao mensur\'avel a respeito da tribo produto
%${\cal S} \times {\cal T}$. Ent\~ao, para cada $x\in X$
%a fun\c c\~ao
%$$
%y\mapsto f(x,y)
%$$
%\'e mensur\'avel a respeito da tribo ${\cal T}$.
%Al\'em disso, se $\nu$ \'e $\sigma$-finita, o conjunto
%$$A:=\{ \, x\in X \, : \, y\in Y \mapsto f(x,y) \
%\mbox{\rm \'e $\nu-$integr\'avel} \, \}$$
%\'e mensur\'avel e a fun\c c\~ao de $A$ em $\bkC$ definida por
%$$
%x\in A \mapsto \int_Y f(x,y)\, {\rm d}\nu(y)
%$$
%\'e mensur\'avel em $A$.
%\end{proposition}
%
%\begin{theorem}
% {\rm ({\bf de Fubini-Lebesgue})} \
%Sejam $(X,{\cal S},\mu)$ e $(Y,{\cal T},\nu)$
%dois espa\c cos mensurados $\sigma$-finitos. Ent\~ao
%\vspace{0.5em}
%
%{\rm (i)} \ existe uma \'unica medida $\mu\times \nu$
%(dita {\sf produto de $\mu$ e $\nu$}) no espa\c co mensur\'avel
%produto $(X\times Y, {\cal S}\times {\cal T})$ que satisfaz a
%condi\c c\~ao
%$$
%(\mu \times \nu)(E\times F)=\mu(E) \, \nu(F)
%$$
%para todo o rect\^angulo mensur\'avel
%$E\times F$ em $X\times Y$.
%\vspace{0.5em}
%
%{\rm (ii)} \ Se $f$ \'e uma fun\c c\~ao complexa em $X\times Y$
%e $\mu\times\nu-$ integr\'avel, ent\~ao a fun\c c\~ao
%$$
%x\in X \mapsto \int_Y f(x,y)\, {\rm d}\nu(y)
%$$
%\'e mensur\'avel e $\mu-$integr\'avel, e tem-se
%$$
%\int_X \left( \int_Y f(x,y)\, {\rm d}\nu(y) \right) \, {\rm d}\mu(x)
%= \int_{X\times Y}  f(x,y)\, {\rm d}(\mu\times \nu)(x,y) \, .
%$$
%
%{\rm (iii)} \ Analogamente,
%se $f$ \'e uma fun\c c\~ao complexa em $X\times Y$
%e $\mu\times\nu-$ integr\'avel, ent\~ao a fun\c c\~ao
%$$
%y\in Y \mapsto \int_X f(x,y)\, {\rm d}\mu(x)
%$$
%\'e mensur\'avel e $\nu-$integr\'avel, e tem-se
%$$
%\int_Y \left( \int_X f(x,y)\, {\rm d}\mu(x) \right) \, {\rm d}\nu(y)
%= \int_{X\times Y}  f(x,y)\, {\rm d}(\mu\times \nu)(x,y) \, .
%$$
%\end{theorem}
%
%Nas aplica\c c\~oes do teorema precedente \'e importante
%verificar se a hip\'otese de $f$ ser $\mu\times\nu-$integr\'avel
%\'e satisfeita. Para isso, \'e \'util o seguinte
%
%\begin{theorem}
% {\rm ({\bf de Tonelli})} \
%Sejam $(X,{\cal S},\mu)$ e $(Y,{\cal T},\nu)$
%dois espa\c cos mensurados $\sigma$-finitos.
%Se $f$ \'e uma fun\c c\~ao mensur\'avel a respeito da tribo produto
%${\cal S}\times {\cal T}$  e n\~ao negativa em $X\times Y$, ent\~ao
%$$
%\begin{array}{rcl}
%\displaystyle
%\int_X \left( \int_Y f(x,y)\, {\rm d}\nu(y) \right) \, {\rm d}\mu(x)
%& = &
%\displaystyle
%\int_Y \left( \int_X f(x,y)\, {\rm d}\mu(x) \right) \, {\rm d}\nu(y)  \\
%\rule{0pt}{2.5em}
%& = &
%\displaystyle
%\int_{X\times Y}  f(x,y)\, {\rm d}(\mu\times \nu)(x,y) \, .
%\end{array}
%$$
%\end{theorem}
%
%\noindent{\bf Observa\c c\~oes:}
%\vspace{0.5em}
%
%1. Decorre do teorema de Tonelli que se $\varphi$ \'e uma
%qualquer fun\c c\~ao mensur\'avel complexa em $X\times Y,$
%e se a fun\c c\~ao
%$g(x):=\int_Y|\varphi(x,y)|\, {\rm d}\nu(y)$
%satisfaz a condi\c c\~ao
%$\int_X g\, {\rm d}\mu <+\infty$
%(ou se a fun\c c\~ao
%$h(y):=\int_X|\varphi(x,y)|\, {\rm d}\mu(x)$
%satisfaz a condi\c c\~ao
%$\int_Y h\, {\rm d}\nu <+\infty$),
%ent\~ao $\varphi$ \'e $\mu\times\nu-$integr\'avel.
%\vspace{0.5em}
%
%2. Os teoremas de Fubini e de Tonelli estendem-se tamb\'em ao caso
%de produtos finitos $X_1\times\ldots\times X_n$ de
%espa\c cos mensurados $\sigma-$finitos.
%
%
%\section{Rela\c c\~oes entre os integrais de Riemann e de Lebesgue.
%Exemplos.}
%
%\hspace{1em}
%Nesta sec\c c\~ao vamos referir alguns resultados que permitem
%relacionar os integrais de Riemann e de Lebesgue, relativamente
%\`a medida de Borel em $\bkR$.
%Note-se, por\'em, que no tocante \`a integra\c c\~ao relativamente
%\`as medidas de Borel e Lebesgue em $\bkR^n$,
%provam-se os seguintes factos:
%\vspace{0.5em}
%
%(i) Se uma fun\c c\~ao $f$ \'e mensur\'avel \`a Borel
%(i.e., relativamente \`a tribo de Borel) -- logo tamb\'em
%mensur\'avel \`a Lebesgue -- ent\~ao \'e integr\'avel \`a
%Borel (i.e., a respeito da medida de Borel) se e s\'o se
%\'e integr\'avel \`a Lebesgue
%(i.e., integr\'avel no sentido de Lebesgue a respeito da medida de Lebesgue),
%e nesse caso os integrais de $f$ s\~ao iguais.
%\vspace{0.5em}
%
%(ii) Se uma fun\c c\~ao $f$ \'e mensur\'avel \`a Lebesgue
%ent\~ao existe uma fun\c c\~ao $f_0$, tal que $f_0=f$ a.e. relativamente \`a
%medida de Lebesgue, que \'e mensur\'avel \`a Borel.
%Consequentemente, se $f$ tamb\'em for integr\'avel \`a
%Lebesgue ent\~ao $f_0$  \'e integr\'avel \`a Borel e os
%integrais de $f$ e $f_0$ relativamente \`as medidas respectivas s\~ao iguais.
%\vspace{0.5em}
%
%\begin{theorem}
%Seja $f$ uma fun\c c\~ao real mensur\'avel \`a Borel e definida
%num intervalo compacto $[a,b]$.
%Suponha-se que $f$ \'e integr\'avel \`a Riemann em $[a,b]$.
%Ent\~ao $f$ \'e tamb\'em integr\'avel \`a Lebesgue relativamente
%\`a medida $\lambda$ de Borel em $[a,b]$
%e os dois integrais coincidem, i.e.,
%$$
%\int_{[a,b]}f \, {\rm d}\lambda =
%\int_a^bf \, .
%$$
%\end{theorem}
%
%\noindent{\bf Observa\c c\~oes:}
%\vspace{0.5em}
%
%1. A condi\c c\~ao de $f$ ser mensur\'avel \`a Borel pode
%dispensar-se. Com efeito, prova-se que sendo $f$ integr\'avel
%\`a Riemann ent\~ao existe uma fun\c c\~ao $g$ mensur\'avel \`a
%Borel tal que $f=g$ $\lambda-$a.e..
%\vspace{0.5em}
%
%2. O rec\'\i proco do teorema n\~ao se verifica em geral, i.e.,
%uma fun\c c\~ao pode ser integr\'avel \`a Lebesgue sem que o
%seja \`a Riemann. Um (contra-)exemplo \'e fornecido pela
%fun\c c\~ao de Dirichlet
%$$
%f(x):=\chi_{\bkQ}(x) \, , \quad x\in [0,1] \, ,
%$$
% a qual n\~ao \'e integr\'avel \`a Riemann
%(como facilmente se constata), mas \'e
%integr\'avel \`a Lebesgue, pois
%$$
%\int_{[0,1]}f \, {\rm d}\lambda =
%\int_{[0,1]} \chi_{\bkQ} \, {\rm d}\lambda =
%\lambda (\bkQ\cap [0,1]) = 0 \,
%$$
%(a \'ultima igualdade \'e justificada pelo facto de a medida de
%Borel de qualquer conjunto numer\'avel ser nula).
%\vspace{0.5em}
%
%3. No caso de $f$ ser n\~ao negativa e cont\'\i nua
%no intervalo $[0,1]$,
%indiquemos aqui, sumariamente, os t\'opicos da demonstra\c c\~ao do
%teorema, a qual pode fazer-se com base
%no teorema da converg\^encia mon\'otona.
%Com efeito, sendo $f$ cont\'\i nua em $[0,1]$,
%sabemos que \'e a\'\i \ integr\'avel
%\`a Riemann e que o integral de Riemann pode calcular-se
%(como limite de somas de Riemann)
%de acordo com a igualdade
%$$
%\int_0^1f = \lim_{n\rightarrow +\infty}
%\, \frac{1}{2^n} \sum_{k=0}^{2^n-1}
%\left( \inf_{x\in I_{k,n}} f(x) \right) \, ,
%\eqno(1)
%$$
%que provem de se considerarem parti\c c\~oes do intervalo $[0,1]$
%em $2^n$ intervalos de igual amplitude $1/2^n$,
% $I_{k,n}:=[\, k/2^n,(k+1)/2^n \, ] $,
%para cada $n\in\bkN$ (fixo) e $k=0,1,\ldots,2^n-1$. Definindo
%$$
%f_n(x):=\sum_{k=0}^{2^n-1}
%\left( \inf_{x\in I_{k,n}} f(x) \right) \,
%\chi_{I_{k,n}}(x)\, ,
%$$
%prova-se que $\{f_n\}_{n\in\bkN}$ \'e uma
%sucess\~ao mon\'otona crescente
%de fun\c c\~oes mensur\'avel simples e n\~ao negativas
%que converge (ascendentemente) para $f$ em $[0,1]$,
%$$
%f_n \uparrow f \quad (n\rightarrow +\infty) \, .
%$$
%Ora, por defini\c c\~ao de integral de Legbesgue de uma
%fun\c c\~ao simples, tem-se
%$$
%\int_{[0,1]}f_n\, {\rm d}\lambda =
%\sum_{k=0}^{2^n-1}
%\left( \inf_{x\in I_{k,n}} f(x) \right) \,
%\lambda(I_{k,n}) =
%\frac{1}{2^n} \sum_{k=0}^{2^n-1}
%\left( \inf_{x\in I_{k,n}} f(x) \right)  \eqno(2)
%$$
%(pois $\lambda(I_{k,n})=1/2^n$).
%Assim, por (1) e (2) e aplicando em seguida o teorema da
%converg\^encia mon\'otona, podemos escrever
%$$
%\int_0^1f = \lim_{n\rightarrow +\infty}
%\int_{[0,1]}f_n\, {\rm d}\lambda =
%\int_{[0,1]}\left( \lim_{n\rightarrow +\infty} f_n \right)
%\, {\rm d}\lambda =
%\int_{[0,1]}f\, {\rm d}\lambda \, ,
%$$
%o que prova o pretendido.
%\vspace{1em}
%
%De acordo com o teorema anterior, podemos afirmar que o integral
%de Lebesgue \'e mais geral que o integral pr\'oprio de
%Riemann, no sentido de que a exist\^encia daquele implica a
%exist\^encia deste, sendo ent\~ao iguais os valores de ambos os
%integrais.
%Por\'em, no caso dos integrais impr\'oprios de Riemann, do tipo
%$$
%\int_{-\infty}^{+\infty}f:=
%\lim_{\stackrel{\scriptstyle a\rightarrow -\infty }{\stackrel{}{
%       \scriptsize b\rightarrow +\infty }}}
%\int_a^b f \, ,
%$$
%isto pode n\~ao suceder.
%O (contra-)exemplo t\'\i pico \'e dado considerando
%a fun\c c\~ao
%$$
%f(x):=\frac{\sin x}{x} \, , \quad x\in\bkR
%$$
%(com $f(0)=1$), para a qual o integral de Lebesgue em
%$\bkR$ n\~ao existe,
%mas $f$ \'e integr\'avel \`a Riemann, tendo-se
%$$
%\int_{-\infty}^{+\infty} \frac{\sin x}{x} \, {\rm d}x=\pi \, .
%$$
%A n\~ao exist\^encia do integral de Lebesgue para esta fun\c c\~ao
%decorre do facto de n\~ao existir
%o integral impr\'oprio no sentido de Riemann da
%fun\c c\~ao $|f|$,
%$x\in\bkR \mapsto  | \sin x | / |x| $, e do seguinte
%
%\begin{theorem}
%Seja $f:\bkR \rightarrow \bkR_0^+$ uma fun\c c\~ao
%mensur\'avel \`a Borel.
%Suponha-se que $f$ \'e integr\'avel \`a Riemann sobre
%todos os intervalos compactos de $\bkR$.
%Ent\~ao, $f$ \'e integr\'avel \`a Lebesgue se e s\'o se
%o integral impr\'oprio de Riemann existir, e nesse caso
%os dois integrais coincidem:
%$$
%\int_{\bkR} f \, {\rm d}\lambda =
%\int_{-\infty}^{+\infty} f \, .
%$$
%\end{theorem}
%
%Mais geralmente, prova-se o seguinte
%
%\begin{theorem}
% {\rm ({\bf de Lebesgue})} \
%Uma fun\c c\~ao $f$ limitada em $[a,b]$ \'e integr\'avel \`a Riemann
%em $[a,b]$ se e s\'o se \'e cont\'\i nua quase em toda a parte
%relativamente \`a medida $\lambda_1$ de Lebesgue em $\bkR$.
%$f$ \'e ent\~ao integr\'avel \`a Lebesgue e os dois integrais coincidem:
%$$
%\int_{[a,b]}f \, {\rm d}\lambda_1 =
%\int_a^bf \, .
%$$
%A propriedade da igualdade dos dois integrais estende-se tamb\'em ao
% caso dos integrais impr\'oprios de Riemann absolutamente convergentes.
%\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Integral de Lebesgue. Teoremas fundamentais.}

\hspace{1em} Se $f$ \'e uma fun\c c\~ao que toma valores em $\mathbb{R}$,
 chama-se
{\sf parte positiva} de $f$ \`a fun\c c\~ao $f^+$ definida por
$$
f^+:=\sup\{ f,0 \} \, ;
$$
analogamente, a {\sf parte negativa} de $f$ \'e a
 fun\c c\~ao $f^-$ definida por
$$
f^-:=-\inf\{ f,0 \} \, .
$$
Constata-se de imediato que
$$
f^+ \geq 0 \, , \quad
f^- \geq 0 \, , \quad
f=f^+-f^- \, , \quad
|f|=f^++f^- \, .
$$
Al\'em disso,
se $f$ \'e mensur\'avel, tamb\'em $f^+$ e $f^-$ o s\~ao.

\begin{definition}
 {\rm {\bf (integral de Lebesgue)}}
 Seja $(X,\mathcal{M},\mu)$ um espa\c co mensurado e
$f$ uma fun\c c\~ao real ou complexa mensur\'avel em $X$.
O {\sf integral de $f$ relativamente a} $\mu$,
$\displaystyle \int_X f{\rm d}\mu$,
define-se de acordo com as seguintes etapas:
\vspace{0.5em}

{\rm (i)} \ se $f$ \'e uma fun\c c\~ao simples, digamos,
$f=\sum_{i=1}^m\alpha_i \chi_{E_i}$, definimos
$$
\int_X f \, {\rm d}\mu := \sum_{i=1}^m \alpha_i \mu(E_i) \, ;
$$

{\rm (ii)} \ se $f$ \'e n\~ao negativa, definimos
$$
\int_X f \, {\rm d} \mu :=
 \sup_{\stackrel{\scriptstyle 0\leq \varphi \leq f}{\stackrel{}{
       \mbox{\scriptsize \rm $\varphi$ simples}}}}
\int_X \varphi \, {\rm d}\mu  \, ;
$$

{\rm (iii)} \ $f$ diz-se {\sf integr\'avel
 (ou som\'avel)  \`a Lebesgue em $X$
relativamente a $\mu$} (ou, simplesmente,
$\mu-${\sf integr\'avel em} $X$) se
$$
\int_X |f| \,{\rm d} \mu <+\infty \, ;
$$

{\rm (iv)} \ se $f$ \'e real e $\mu-$integr\'avel, definimos
$$
\int_X f \, {\rm d} \mu :=
 \int_X f^+ \, {\rm d}\mu -
\int_X f^- \, {\rm d}\mu \, ;
$$

{\rm (v)} \ se $f$ \'e complexa e $\mu-$integr\'avel, digamos,
$f = f_r+if_i$,
definimos
$$
\int_X f \, {\rm d} \mu :=
 \int_X f_r \, {\rm d}\mu +
i \int_X f_i \, {\rm d}\mu \, .
$$
\end{definition}

\noindent{\bf Observa\c c\~oes:}
\vspace{0.5em}

1. O integral de uma fun\c c\~ao mensur\'avel
 n\~ao negativa existe sempre -- pode \'e ser infinito!.
Al\'em disso, quando $f\geq0$ em $X$, \'e usual escrever
$\int_X f \, {\rm d}\mu=+\infty$ para indicar que
$f$ n\~ao \'e $\mu-$integr\'avel sobre $X$.
\vspace{0.5em}

2. Resulta imediatamente da defini\c c\~ao que uma fun\c c\~ao
mensur\'avel $f$ \'e integr\'avel \`a Lebesgue
se e s\'o se $|f|$ o for. Recorde-se que isto n\~ao sucede no
caso do integral de Riemann.
\vspace{0.5em}

3. Quando $\mu=\lambda_n$ \'e a medida de Lebesgue, normalmente escreve-se
$\displaystyle \int_X f {\rm d}x_1 \ldots {\rm d}x_n$ ou,
simplesmente, $\displaystyle \int_X f{\rm d}x$,
em vez de
$\displaystyle \int_X f{\rm d}\lambda_n$.
\vspace{0.5em}

4. Como se sabe, na defini\c c\~ao de integral de Riemann
consideram-se parti\c c\~oes do dom\'\i nio da fun\c c\~ao.
Por\'em, na defini\c c\~ao do integral de Lebesgue estamos
sobretudo interessados nos valores que a fun\c c\~ao
assume, i.e., no contradom\'\i nio da fun\c c\~ao --
em certo sentido, podemos dizer que no
integral de Lebesgue se
consideram parti\c c\~oes do contradom\'\i nio da fun\c c\~ao.
\vspace{0.5em}

O resultado central na Teoria do Integral de Lebesgue \'e,
sem d\'uvida, o seguinte

\begin{theorem}
{\rm {\bf (da converg\^encia dominada de Lebesgue)}} \
Seja $(X,\mathcal{M},\mu)$ um espa\c co mensurado e $\{f_n\}_{n\in\mathbb{N}}$
uma sucess\~ao de fun\c c\~oes complexas e $\mu-$mensur\'aveis em $X$.
Suponha-se que
$$
\begin{array}{cl}
{\rm (i)} & f_n\rightarrow 0 \quad \mbox{\rm a.e. em $X$}  \\
\rule{0pt}{1.2em}
{\rm (ii)} & \mbox{\rm existe uma fun\c c\~ao $g$ que \'e $\mu-$integr\'avel em $X$ e tal que}
\end{array}
$$
$$
|f_n|\leq g \quad \mbox{\rm a.e. em $X$, \ para todo o $n\in\mathbb{N}$} \, .
$$
Nestas condi\c c\~oes, $f_n$ e $f$ s\~ao $\mu-$integr\'aveis em $X$ e
$$
\int_X f \, {\rm d}\mu =
\lim_{n\rightarrow +\infty} \, \int_{X}f_n \, {\rm d}\mu \, .
$$
\end{theorem}



==> opsf_t10_2016-17.tex <==


%\chapter{What is the arithmetic nature of $\zeta(2k+1)\;$?}

\chapter{Ap\'ery Theorem}

\pagestyle{myheadings}\markright{What is the arithmetic nature of $\zeta(2k+1)\;$?}
\pagestyle{myheadings}\markleft{J. Petronilho}


\section{Remarks on Ap\'ery's proof of $\zeta(3)\not\in\mathbb{Q}$}

%referir o problema de basel

Consider the {\sl Riemann zeta function}
\begin{snugshade}
$$
\zeta(s):=\sum_{n=1}^\infty \frac{1}{n^s}\,,\quad \Re s>1\;.
$$
\end{snugshade}
\noindent
It is known (since Euler!) that when $s=2k$ is an even positive integer number, then
\begin{snugshade}
$$
\zeta(2k)=\frac{(-1)^{k-1}2^{2k-1}B_{2k}}{(2k)!} \,\pi^{2k}
$$
\end{snugshade}
\noindent
($k\in\mathbb{N}$), where the $B_n$'s are the so-called {\sl Bernoulli numbers}, defined by
\begin{snugshade}
$$
\frac{x}{e^x-1}=\sum_{n=0}^{\infty}B_n\frac{x^n}{n!}\;.
$$
\end{snugshade}
\noindent
Note that
$B_0=1$, $B_1=-\frac{1}{2}$, $B_2=\frac{1}{6}$, $B_4=-\frac{1}{30}$, $B_6=\frac{1}{42}$, $B_8=-\frac{1}{30}$,  $B_{10}=\frac{5}{66}$, etc., being $B_{2k+1}=0$ and $B_{2k}\in\mathbb{Q}$ for each $k\in\mathbb{N}$.
Therefore, recalling that $\pi$ is a transcendental number (a fact proved by Lindemann in 1882), it follows that
\begin{snugshade}
$$
\zeta(2k)\not\in\mathbb{Q}
$$
\end{snugshade}
\noindent
($k\in\mathbb{N}$). The case of the odd zeta values, i.e., to determine the arithmetic nature of $\zeta(2k+1)$,
is surprisingly much more intricate.
It was only in 1978 that the French mathematician Roger Ap\'ery \ref{Apery1979} proved that $\zeta(3)\not\in\mathbb{Q}$.
Ap\'ery presented his proof at the {\it Journ\'ees Arithm\'etiques de Marseille-Luminy} (June 1978).
His proof was so miraculous that it produced a widespread scepticism in the audience.
In an attempt to explain it, about two months after Ap\'ery's presentation,
Henry Cohen delivered a lecture (at the International Congress of Mathematics, in Helsinkin)
giving full details of the proof, based on his discussions with Hendrik Lenstra and Alfred van der Poorten.
An informal presentation of all this appears in \ref{Poorten1979}.
However, a simpler proof was given by Fritz Beukers \ref{Beukers1979}
in the meantime between the meetings at Luminy and Helsinki.
%about two months after Ap\'ery's presentation.
We will give full details of Beukers's proof in the next section.
For the moment, we summarize Ap\'ery's proof
of the irrationality of $\zeta(3)$, without going into the details.

Consider the recurrence relation
\begin{snugshade}
$$
n^3u_n+(n-1)^3u_{n-2}=(34n^3-51n^2+27n-5)u_{n-1} \; , \quad n\geq2\;,
$$
\end{snugshade}
\noindent
and then introduce two sequences $\{a_n\}_{n\geq0}$ and $\{b_n\}_{n\geq0}$ as
\begin{snugshade}
$$
\begin{array}{ccccc}
a_0=0 & ; & a_1=6 & ; & a_n=u_n \; , \; n\geq2\\
b_0=1 & ; & b_1=5 & ; & b_n=u_n \; , \; n\geq2\,.
\end{array}
$$
\end{snugshade}
\noindent
Ap\'ery proved that $a_n$ and $b_n$ are explicitly determined by
\begin{snugshade}
$$
a_n = \sum_{k=0}^{n}\mbox{$\binom{n}{k}^2\binom{n+k}{k}^2$}c_{n,k} \; , \quad
b_n = \sum_{k=0}^{n}\mbox{$\binom{n}{k}^2\binom{n+k}{k}^2$}\;,\quad n\in\mathbb{N}_0\;,
$$
\end{snugshade}
\noindent
where, for each $n\in\mathbb{N}_0$ and $k\in\{0,1,\ldots,n\}$,
$$
c_{n,k} := \sum_{m=1}^{n}\frac{1}{m^3} + \sum_{m=1}^{k}\frac{(-1)^{m-1}}{2m^3\binom{n}{m}\binom{n+m}{m}}\;.
$$
Clearly, $c_{n,k}\to\zeta(3)$ as $n\to+\infty$ (for each fixed $k\in\mathbb{N}$),
from which we may prove that (see e.g. \ref{Butler2015}, Lemma 4)
$$
\frac{a_n}{b_n}\to\zeta(3)\;.
$$
Moreover, the convergence is so fast that,
denoting by $d_n$ the least common multiple of the numbers $1,2,\ldots,n$,
and setting\vspace*{-0.5em}
\begin{snugshade}
$$
A_n:=2d_n^3a_n\in\mathbb{Z}\;,\quad B_n:=2d_n^3b_n\in\mathbb{N}
$$
\end{snugshade}
\noindent
(so that we still have $A_n/B_n\to\zeta(3)$ as $n\to+\infty$), then\vspace*{-0.5em}
\begin{snugshade}
$$
0\neq \big| A_n-B_n\zeta(3) \big| \to 0\;,\quad\mbox{\rm as}\quad n\to+\infty\;.
$$
\end{snugshade}
\noindent
Thus indeed Ap\'ery established the irrationality of $\zeta(3)$, according with the following

\begin{snugshade}
\begin{lemma}\label{crit-irrational}
Let $\zeta\in\mathbb{R}$.
Suppose that there exist sequences of integer numbers
$\{ A_n\}_{n \in \mathbb{N}}$ and $\{B_n\}_{n\in\mathbb{N}}$
such that the following two conditions hold:
\begin{enumerate}
\item[{\rm (i)}] $A_n+\zeta B_n\neq0$ for each $n\in\mathbb{N}$; \vspace*{0.25em}
\item[{\rm (ii)}] $\big| A_n+\zeta B_n\big| \to 0$ as $n\to\infty$.
\end{enumerate}
Then $\zeta\not\in\mathbb{Q}$.
\end{lemma}
\end{snugshade}

{\it Proof.}
Suppose that $\zeta\in\mathbb{Q}$.
Then $\zeta=\frac{p}{q}$ for some integer numbers $p\in\mathbb{Z}$ and $q\in\mathbb{N}$.
Using the hypothesis (i) and (ii), we may write
$$
0<\frac{1}{q}\leq \frac{| qA_n+pB_n|}{q}=\left|A_n+\zeta B_n\right|\to0\;,\quad\mbox{\rm as}\;\; n\to\infty\;.
$$
Since we obtained a contradiction, we may conclude that $\zeta\not\in\mathbb{Q}$.
\qed


\section{Preliminaries on Number Theory}

Consider the function $\pi:\mathbb{R}\to\mathbb{N}_0$ defined by
\begin{snugshade}\vspace*{-0.5em}
\begin{equation}\label{pix-def}
%\pi(x):=\mbox{\rm number of prime numbers less than or equal to $x$}\;.
\pi(x):=\sharp\big\{\,p\,|\,\mbox{\rm $p$ is a prime number and $p\leq x$}\,\big\}
\end{equation}
\end{snugshade}
\noindent
(so that $\pi(x)$ is the number of prime numbers less than or equal to $x$).
The Prime Number Theorem of Hadamard and la Vall\'e Poussin (1896) states that:\vspace*{-.5em}
\begin{snugshade}
\begin{equation}\label{pixPNT}
\lim_{x\to+\infty}\,\frac{\pi(x)}{x/\ln x}=1\; .
%\lim_{x\to+\infty}\frac{\;\;\pi(x)\;\;}{\rule{0pt}{1.25em}\displaystyle\frac{x}{\ln x}}=1\; .
\end{equation}
\end{snugshade}
\noindent
We will use this result to obtain some useful estimates for the least common multiple (l.c.m.) of the numbers $1,2,\ldots,n$ ($n\in\mathbb{N}$), which will be denoted by $d_n$. First we notice that $d_n$ admits the following representation:\vspace*{-.5em}
\begin{snugshade}
\begin{equation}\label{f1-LCM}
d_n:=\mbox{\rm l.c.m.}\{1,2,\cdots,n\}
=\prod_{\substack{p\leq n \\ \mbox{\rm\scriptsize $p$ prime}}}p^{\lfloor\ln n/\ln p\rfloor}\;.
\end{equation}
\end{snugshade}
\noindent
Indeed, for each prime number $p\leq n$, let $r$ be the greatest positive integer number such that $p^r\leq n$.
Clearly, $r=\lfloor\ln n/\ln p\rfloor\,$, hence equality (\ref{f1-LCM}) follows taking into account the
well known characterization of the least common multiple by prime factorization.\footnote{\,Such characterization is a consequence of the Fundamental Theorem of Arithmetics, and it asserts that, given $k$ positive integer numbers $n_1,n_2,\ldots,n_k$, then l.c.m.$\{n_1,n_2,\ldots,n_k\}$ is obtained multiplying all the highest powers of each prime number among all the powers of prime numbers appearing in the factorizations of each of the numbers $n_1,n_2,\ldots,n_k$.}
%From (\ref{f1-LCM}) and (\ref{pixPNT}) one easily see that,
Furthermore, for each $\epsilon>0$ there exists $n_0=n_0(\epsilon)\in\mathbb{N}$ such that
\begin{snugshade}\vspace*{-.5em}
\begin{equation}\label{f2-LCM}
d_n\leq n^{\pi(n)}<e^{(1+\epsilon)n}\quad\mbox{\rm if}\quad n\geq n_0(\epsilon)\;.
\end{equation}
\end{snugshade}
\noindent
(The first inequality holds really for all $n\in\mathbb{N}$.)
In fact, on the first hand, from (\ref{f1-LCM}) we deduce
%\begin{snugshade}
$$%begin{equation}\label{f2-LCM}
d_n\leq\prod_{\substack{p\leq n \\ \mbox{\rm\scriptsize $p$ prime}}}p^{\ln n/\ln p}
=\prod_{\substack{p\leq n \\ \mbox{\rm\scriptsize $p$ prime}}}p^{\log_p n}
=\prod_{\substack{p\leq n \\ \mbox{\rm\scriptsize $p$ prime}}}n
=n^{\pi(n)}\;.
$$%<n^{\pi(n)}<3^n\quad \mbox{\rm (for $n$ sufficiently large)}\; ,
%\end{equation}
%\end{snugshade}
%\noindent
On the other hand, from (\ref{pixPNT}), given $\epsilon>0$,
there exists $n_0=n_0(\epsilon)\in\mathbb{N}$ such that
$\pi(n)<(1+\epsilon)n/\ln n$ for each $n\geq n_0$,
%$$
%\pi(n)<\frac{(1+\epsilon)n}{\ln n}\quad\mbox{\rm if}\;\; n\geq n_0\; ,
%$$
hence the last inequality in (\ref{f2-LCM}) follows: % by noticing that, for each $n\geq n_0$,
$$
n^{\pi(n)}%=e^{\ln\big(n^{\pi(n)}\big)}
=e^{\pi(n)\ln n}<e^{(1+\epsilon)n}\quad\mbox{\rm if}\quad n\geq n_0\;.
$$
%This proves the last inequality in (\ref{f2-LCM}), by choosing $\epsilon=\ln3-1$.

\begin{remark}\em
Taking $\epsilon:=\ln3-1$ in (\ref{f2-LCM}), we obtain the useful estimate
\begin{snugshade}\vspace*{-.5em}
$$%\begin{equation}\label{f3-LCM}
d_n<3^{n}\quad\mbox{\rm for $n$ sufficiently large}\;.
$$%\end{equation}
\end{snugshade}
\end{remark}

\begin{remark}\em
Estimates of the form
\begin{snugshade}%\vspace*{-.5em}
$$
a\,\frac{n}{\ln n}<\pi(n)<b\,\frac{n}{\ln n}\quad\mbox{\rm for $n$ sufficiently large}\;,
$$
\end{snugshade}
\noindent
where $a$ and $b$ are (absolute) constants independent of $n$,
were first discovered by P. L. Chebychev around 1852, who gave the values $a=0.92$ and $b=1.11$.
It is worth mentioning that such estimate avoid the use of the Prime Number Theorem
in the proof of the irrationality of $\zeta(3)$, as we will see in the next section.
\end{remark}

\section{Beukers's proof of $\zeta(3)\not\in\mathbb{Q}$}



\section{Remarks and historical notes}




\section*{Exercises}
%\bigskip

%\noindent
\begin{enumerate}[label=\emph{\bf \arabic*.},leftmargin=*]
\item Prove that the Bernoulli numbers, defined by (\ref{}), satisfy the recurrence relation...
\medskip

%\item
%Sejam $X$ um e.v. real, $p:X\rightarrow\mathbb{R}$ uma funcional sublinear e
%$K:=\{\,x\in X\,|\, p(x)<1\,\}\,$. Mostre que: % $K$ satisfaz as propriedades seguintes:
%\begin{enumerate}
%\item $K$ \'e convexo;
%\item $0$ \'e um ponto interior de $K$ (no sentido da Defini\c c\~ao \ref{def-pontoInt});%(no sentido alg\'ebrico).
%\item $p$ \'e a funcional de Minkowski do conjunto $K$.
%\end{enumerate}
%\medskip

\item
Ex 3
\end{enumerate}
\bigskip

%\medskip

\section*{Bibliography}
%\medskip

{\small
\begin{enumerate}[label=\emph{\rm [\arabic*]},leftmargin=*]
\item\label{Poorten1979} A. van der Poorten, A proof that Euler missed... Ap\'ery's proof of the irrationality of $\zeta(3)$,
          {\it The Mathematical Intelligencer} {\bf 1} (4) (1979) 195--203.
\item\label{Apery1979} R. Ap\'ery, Irrationalit\'e de $\zeta(2)$ et $\zeta(3)$,
          {\it Ast\'erisque} {\bf 61} (1979) 11--13.
\item\label{BallRivoal2000} K. Ball and T. Rivoal, Irrationalit\'e d'une infinit\'e de valeurs
de la fonction z\^eta aux entiers impairs,
          {\it Invent. Math.} {\bf 146} (2001) 193--207.
\item\label{Beukers1979} F. Beukers, A note on the irrationality of $\zeta(2)$ and $\zeta(3)$,
          {\it Bull. London Math. Soc.} {\bf 11} (1979) 268--272.
\item\label{Butler2015} L. A. Butler, A useful application of Brun's irrationality criterion,
          {\it Expo. Math.} {\bf 33} (2015) 121--134.
\item\label{Zudilin2001} W. V. Zudilin, One of the numbers $\zeta(5),\zeta(7),\zeta(9),\zeta(11)$ is irrational,
{\it Uspekhi Mat. Nauk.} [{\it Russian Math. Surveys}] {\bf 56} (2001) (4) 149--150.
\end{enumerate}
}



==> opsf_t11_2016-17.tex <==


\chapter{Spectral theorem for unitary operators}

\pagestyle{myheadings}\markright{Spectral theorem for unitary operators}
\pagestyle{myheadings}\markleft{J. Petronilho}

One of the most important results in Analysis is the Spectral Theorem, which
states the connection between linear operators on a Hilbert space and measures.
Indeed, this fundamental result illustrates a strong connection between
algebraic objects (linear operators) and analytic objects (measures).
Such connection is a powerful idea in mathematics as it allows us to use tools
from one area of mathematics to obtain conclusions in another area.
For our purposes, the reader should keep in mind that several of the most
powerful results appearing in the framework of OPUC
will be rooted in this connection.
In these notes we will establish the Spectral Theorem as a direct consequence
of Herglotz Theorem. In order to state this last theorem
we need the concept of positive-definite sequence, as well as some basic properties of such sequences.


\section{Positive-definite sequences}


\begin{snugshade}
\begin{definition}
A sequence of numbers $(c_n)_{n\in\mathbb{Z}}\subset\mathbb{C}$
is called {\sl positive-definite} if
\begin{equation}\label{posit-seq1}
\sum_{n,m=0}^Nc_{n-m}a_n\overline{a}_m\geq0\; ,
\quad\forall(a_n)_{n\in\mathbb{N}_0}\subset\mathbb{C}\;,\;\forall N\in\mathbb{N}_0\; .
\end{equation}
\end{definition}
\end{snugshade}
\noindent
The following proposition lists some basic properties of positive-definite sequences.

\begin{snugshade}
\begin{proposition}\label{prop-posit-seq1}
Let $(c_n)_{n\in\mathbb{Z}}$ be a positive-definite sequence. % in $\mathbb{C}$.
Then: \smallskip %the following properties hold:
$$
\begin{array}{rl}
\mbox{\rm (i)} & c_0\big(|a|^2+|b|^2\big)+c_n\overline{a}b+c_{-n}a\overline{b}\geq0\;,\;
\forall n\in\mathbb{Z}\; ,\; \forall a,b\in\mathbb{C}\; ; \\ [0.6em]
\mbox{\rm (ii)} & c_{-n}=\overline{c_n}\; ,\; \forall n\in\mathbb{Z}\; ;\\ [0.6em]
\mbox{\rm (iii)} & |c_{n}|\leq c_0\; ,\; \forall n\in\mathbb{Z}\; .
\end{array}
$$
\end{proposition}
\end{snugshade}

{\it Proof.}
(i)
Taking $N=0$ and $(a_n)_{n\in\mathbb{N}_0}=(1,0,0,0,\cdots)$ in (\ref{posit-seq1}),
we obtain $c_0\geq0$.
Hence, for $n=0$, the left-hand side of the inequality in (i) becomes
$$
c_0\big(|a|^2+|b|^2+\overline{a}b+a\overline{b}\,\big)=c_0|a+b|^2\geq0\; ,
$$
and so the inequality in (i) is true for $n=0$.
Next, fix $N\in\mathbb{N}$ and choose $(a_n)_{n\in\mathbb{N}_0}$ such that
%$$%\begin{equation}\label{escolhaA1}
%a_0:=a\; ,\quad a_N:=b\, ,\quad a_n:=0\;\mbox{\rm if}\; n\neq0,N\; .
%$$%\end{equation}
$a_0:=a$, $a_N:=b$, and $a_n:=0$ if $n\neq0,N$.
Then, from (\ref{posit-seq1}),
%$$
%\begin{array}{rcl}
%\displaystyle 0\leq\sum_{n,m=0}^Nc_{n-m}a_n\overline{a}_m
%&=& \displaystyle\sum_{n,m\in\{0,N\}}c_{n-m}a_n\overline{a}_m \\ [2em]
%&=& c_0\big(|a_0|^2+|a_N|^2\,\big)+c_N\overline{a_0}a_N+c_{-N}a_0\overline{a_N}\\ [1em]
%&=&c_0\big(|a|^2+|b|^2\,\big)+c_N\overline{a}b+c_{-N}a\overline{b}\; ,
%\end{array}
%$$
$$
0\leq\sum_{n,m\in\{0,N\}}c_{n-m}a_n\overline{a}_m
=c_0\big(|a|^2+|b|^2\,\big)+c_N\overline{a}b+c_{-N}a\overline{b}\; ,
$$
and this proves the inequality in (i) for $n\in\mathbb{N}$.
Replacing $a$ by $\overline{a}$ and $b$ by $\overline{b}$ in the
inequality in (i) for positive $n$ (already proved)
one realizes that it also remains true for negative $n$.
\smallskip

(ii)
Taking $a=1$ in (i), one has
$c_0\big(1+|b|^2\big)+c_nb+c_{-n}\overline{b}\geq0$
for every $n\in\mathbb{Z}$ and $b\in\mathbb{C}$,
hence, since $c_0\geq0$, we deduce
$$
c_nb+c_{-n}\overline{b}\in\mathbb{R}\;,\quad
\forall n\in\mathbb{Z}\; ,\; \forall b\in\mathbb{C}\;.
$$
Therefore, choosing successively $b=1$ and $b=i$, we see that there exist
sequences of real numbers $(r_n)_n$ and $(s_n)_n$ such that (resp.)
$$
c_n+c_{-n}=r_n\; ,\quad c_n-c_{-n}=is_n\;,\quad\forall n\in\mathbb{Z}\; .
$$
Adding and subtracting both sides of these equalities, we deduce the relations
$$
c_n=\frac{r_n-is_n}{2}\;,\quad c_{-n}=\frac{r_n+is_n}{2}\;,\quad\forall n\in\mathbb{Z}\; .
$$
Therefore, $\overline{c_n}=c_{-n}$ for every $n\in\mathbb{Z}$, and (ii) is proved.
\smallskip

(iii)
Fix $n\in\mathbb{N}$.
In the inequality (i) choose $a=1$ and $b=x\overline{c_n}$, with $x\in\mathbb{R}$.
Then, and taking into account (ii) ---so that $c_{-n}c_n=\overline{c_n}c_n=|c_n|^2$---, we deduce
\begin{equation}\label{eq-quadr-cn}
c_0|c_n|^2\, x^2+2|c_n|^2\,x+c_0\geq0\;,\quad\forall x\in\mathbb{R}\;.
\end{equation}
If $c_0=0$ then $2|c_n|^2\,x\geq0$ for all $x\in\mathbb{R}$,
and this is possible only if $c_n=0$. Thus, by varying $n$, %we see that
(iii) holds trivially if $c_0=0$. If $c_0\neq0$, then in
(\ref{eq-quadr-cn}) we have a quadratic expression in $x$ which is never negative,
hence its discriminant must be non-positive, i.e.,
$\Delta\leq0$, being
$$
\Delta:=\big(|c_n|^2\big)^2-c_0^2|c_n|^2=|c_n|^2\big(|c_n|^2-c_0^2\,\big)\,.
$$
%Henceforth, since
Since $c_0>0$, we see that $\Delta\leq0$ if and only if
$|c_n|\leq c_0$, which proves (iii).
\qed

\begin{remark}\label{c0=1} \em
%We emphasize that
Property (iii) in Proposition \ref{prop-posit-seq1} asserts that
any positive-definite sequence $(c_n)_{n\in\mathbb{Z}}$ is bounded, and $c_0\geq0$.
Moreover, if $c_0=0$ then $c_n=0$ for all $n\in\mathbb{Z}$,
i.e., $(c_n)_{n\in\mathbb{Z}}$ is the trivial (null) sequence.
Therefore, a non-trivial positive-definite sequence must satisfy $c_0\neq0$
($\Leftrightarrow c_0>0$).
Henceforth, without lost of generality, when considering non-trivial
positive-definite sequences, often we will consider $c_0=1$.
\end{remark}

\begin{remark} \em
It follows from (\ref{posit-seq1}) and property (iii) in Proposition \ref{prop-posit-seq1}
that if $(c_n)_{n\in\mathbb{Z}}$ is a positive-definite sequence, then the matrix of order $N+1$
$$
T^{(N+1)}:=\left(
\begin{array}{cccccc}
c_0 & c_1 & c_2 & \cdots & c_{N-1} & c_N \\ [0.25em]
c_{-1} & c_0 & c_1 & \cdots & c_{N-2} & c_{N-1} \\ [0.25em]
c_{-2} & c_{-1} & c_0 & \cdots & c_{N-3} & c_{N-2} \\ [0.25em]
\vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\ [0.25em]
c_{-N+1} & c_{-N+2} & c_{-N+3} & \cdots & c_{0} & c_{1} \\ [0.25em]
c_{-N} & c_{-N+1} & c_{-N+2} & \cdots & c_{-1} & c_{0}
\end{array}
\right)
$$
is an Hermitean and positive-definite matrix for every $N\in\mathbb{N}_0$.
Moreover, $T^{(N+1)}$ is a Toeplitz matrix (i.e., its entries along each diagonal are constants).
\end{remark}


\section{Herglotz Theorem}

As usual, the unit circle will be denoted by $\partial\mathbb{D}:=\{z\in\mathbb{C}:|z|=1\}$,
and we consider its standard parametrization:
$$
z\in\partial\mathbb{D}\quad\Leftrightarrow\quad z=e^{i\theta}\; ,\quad 0\leq\theta<2\pi\; .
$$
Thus, a measure $\mu$ on the unit circle $\partial\mathbb{D}$ will be identified
with a positive Borel measure, still denoted by $\mu$, supported on the interval $[0,2\pi]$.
Accordingly, we will write
\begin{snugshade}
\begin{equation}\label{measUnitCircle}
\int_{\partial\mathbb{D}} f(z)\,{\rm d}\mu(z):=\int_0^{2\pi}f\big(e^{i\theta}\big)\,{\rm d}\mu(\theta)\; ,\quad
\forall f\in L^1\big(\partial\mathbb{D},\mu\big)\; ,
\end{equation}
\end{snugshade}
\noindent
where we implicitly make the identification
\begin{snugshade}
$$
L^1\big(\partial\mathbb{D},\mu\big)\equiv L^1\big([0,2\pi],\mu\big)\; ,
$$
\end{snugshade}
\noindent
in the following sense: being $f:\partial\mathbb{D}\to\mathbb{C}$, then
\begin{snugshade}
$$
f\in L^1\big(\partial\mathbb{D},\mu\big)\quad\Leftrightarrow\quad
f\big(e^{i\theta}\big)\in L^1\big([0,2\pi],\mu\big)\quad\Leftrightarrow\quad
\int_0^{2\pi}\big|f\big(e^{i\theta}\big)\big|\,{\rm d}\mu(\theta)<\infty\;.
$$
\end{snugshade}

\begin{remark} \em
We emphasize that equality (\ref{measUnitCircle}) is an useful convention (definition),
but the reader should keep in mind that it is not obtained by making the change of variables
$z=e^{i\theta}$ in the first integral. For instance, if ${\rm d}\mu(z)={\rm d}z$
(the normalized Lebesgue measure on $\partial\mathbb{D}$), so that
${\rm d}\mu(\theta)=\frac{{\rm d}\theta}{2\pi}$, then
\begin{equation}\label{int-zn1}
\int_{\partial\mathbb{D}} z^n\,{\rm d}z
:=\mbox{$\frac{1}{2\pi}$}\int_0^{2\pi} e^{in\theta}\,{\rm d}\theta
=\left\{\begin{array}{ccl}
1 & \mbox{\rm if} & n=0 \\ [0.25em]
0 & \mbox{\rm if} & n\neq0\; ,
\end{array}\right.
\end{equation}
despite the fact that the change of variables $z=e^{i\theta}$ in the left-hand side integral,
interpreted as an integral of a complex variable function (so that
${\rm d}z=ie^{i\theta}{\rm d}\theta$), would produce the integral
%$\int_{\partial\mathbb{D}} z^n\,{\rm d}z=i\int_0^{2\pi} e^{i(n+1)\theta}\,{\rm d}\theta$.
$i\int_0^{2\pi} e^{i(n+1)\theta}\,{\rm d}\theta$ ($=2\pi i$ if $n=-1$, and $=0$ if $n\neq-1$)
on the right-hand side!
\end{remark}

\begin{snugshade}
\begin{theorem}[Herglotz]\label{Herglotz-Thm}
Let $(c_n)_{n\in\mathbb{Z}}$ be a positive-definite sequence in $\mathbb{C}$.
Then, there exists a unique finite non-negative measure $\mu$ on the unit circle
%$\partial\mathbb{D}:=\{z\in\mathbb{C}:|z|=1\}$
$\partial\mathbb{D}$ ---or, equivalently, a measure on the interval $[0,2\pi]$--- such that
\begin{equation}\label{cn-int1}
c_n=\int_{\partial\mathbb{D}}z^n\,{\rm d}\mu(z)
:=\int_0^{2\pi}e^{in\theta}\,{\rm d}\mu(\theta)\; ,\quad\forall n\in\mathbb{Z}\,.
\end{equation}
Conversely, if $\mu$ is a finite non-negative measure on $\partial\mathbb{D}$,
then  $(c_n)_{n\in\mathbb{Z}}$ defined by $(\ref{cn-int1})$ is
a positive-definite sequence in $\mathbb{C}$.
\end{theorem}
\end{snugshade}

{\it Proof.}
(i) We first prove the existence of $\mu$ satisfying (\ref{cn-int1}).
Without lost of generality we may assume $c_0=1$ (cf. Remark \ref{c0=1}).
Take
$$
0<s<1\; ,\quad z\in\partial\mathbb{D}\; .
$$
Define a sequence $(a_n)_{n\in\mathbb{N}_0}$ by $a_n:=(s/z)^n$.
Then, since $1/\overline{z}=z$, we see that
$$
a_n\overline{a_m}=s^{n+m}z^{m-n}\, ,\quad\forall n,m\in\mathbb{N}_0\; .
$$
Therefore, from (\ref{posit-seq1}), we deduce, for every $N\in\mathbb{N}_0$,
$$
\begin{array}{rcl}
0 & \leq & \displaystyle
\sum_{n,m=0}^Nc_{n-m}s^{n+m}z^{m-n}=\Big|\sum_{n,m=0}^Nc_{n-m}s^{n+m}z^{m-n}\Big|
\leq\sum_{n,m=0}^N|c_{n-m}|\,s^{n+m}\,|z|^{m-n}\\ [2em]
& \leq & \displaystyle\sum_{n,m=0}^Ns^{n+m}=\Big(\sum_{n=0}^Ns^{n}\Big)\Big(\sum_{m=0}^Ns^{m}\Big)
=\Big(\frac{1-s^{N+1}}{1-s}\Big)^2<\frac{1}{(1-s)^2}
\end{array}
$$
(in the third inequality, we have used $|c_{n-m}|\leq c_0=1$), so that, letting $N\to+\infty$,
\begin{equation}\label{seriefsn1}
0\leq f_s(z):=\sum_{n,m=0}^{+\infty}c_{n-m}s^{n+m}z^{m-n}\leq\frac{1}{(1-s)^2}\; ,\quad
0<s<1\;,\; \quad z\in\partial\mathbb{D}\; .
\end{equation}
Notice that these inequalities also show that the series defining $f_s(z)$ is absolutely convergent.
Therefore, we may write
$$
f_s(z) = \sum_{n=0}^{+\infty}\Big(\sum_{m=0}^{+\infty} c_{n-m}s^{n+m}z^{m-n} \Big)
=\sum_{n=-\infty}^{+\infty} c_n z^{-n} \sum_{m=0}^{+\infty} s^{|n|+2m}
=\sum_{n=-\infty}^{+\infty} c_n z^{-n} \frac{s^{|n|}}{1-s^2}
$$
(to see that the second equality holds, write the sum in the left-hand side as
an array---where the entries in each row of this array are the terms of the
sum inside brackets, so that its columns are obtained
by varying $n$---, and then rewrite the sum %(of the entries of all the terms in the array)
by adding the entries along the diagonals of the array), hence
\begin{equation}\label{seriefsn2}
0\leq f_s(z)=\sum_{n=-\infty}^{+\infty} c_n z^{-n} \frac{s^{|n|}}{1-s^2}\; ,
\quad 0<s<1\;,\quad z\in\partial\mathbb{D}\;.
\end{equation}
Therefore,
\begin{equation}\label{intDs1}
\int_{\partial\mathbb{D}}f_s(z)z^{-k}\,{\rm d}z
=\sum_{n=-\infty}^{+\infty} c_n \frac{s^{|n|}}{1-s^2}
 \int_{\partial\mathbb{D}}z^{-n-k}\,{\rm d}z
=c_{-k} \frac{s^{|k|}}{1-s^2}\; ,\quad 0<s<1\;,\; k\in\mathbb{Z}\; ,
\end{equation}
the last equality being justified by (\ref{int-zn1}).
For fixed $s$ ($0<s<1$), we may define an absolutely continuous
measure in $\partial\mathbb{D}$, $\mu_s$, with density
$$
\frac{{\rm d}\mu_s}{{\rm d}z}:=(1-s^2)f_s(z)\; ,\quad z\in\partial\mathbb{D}\;.
$$
Then, from (\ref{intDs1}),
\begin{equation}\label{mu-s1}
\int_{\partial\mathbb{D}}z^{-k}\,{\rm d}\mu_s
=c_{-k} s^{|k|}\; ,\quad 0<s<1\;.
\end{equation}
In particular, for $k=0$,
$$
\mu_s\big(\partial\mathbb{D}\big)=c_0=1\;.
$$
Next, choose a sequence $(s_m)_{m\in\mathbb{N}_0}$, such that
$$
0<s_m<1\; ,\qquad s_m\to1\quad (m\to+\infty)\; .
$$
Then, by (\ref{mu-s1}),
\begin{equation}\label{mu-s2}
\int_{\partial\mathbb{D}}z^{-k}\,{\rm d}\mu_{s_m}
=c_{-k} s_m^{|k|}\quad \xrightarrow{m\to+\infty}\quad c_{-k}
 \; ,\quad \forall k\in\mathbb{Z}\;.
\end{equation}
Therefore, $\int_{\partial\mathbb{D}}p(z)\,{\rm d}\mu_{s_m}$ converges as $m\to+\infty$,
for every (finite) linear combination $p(z)$ of functions of the form $z^k$ ($k\in\mathbb{Z}$);
and since the set of all such functions is dense in $\mathcal{C}\big(\partial\mathbb{D}\big)$,
we conclude that $\int_{\partial\mathbb{D}}f(z)\,{\rm d}\mu_{s_m}$ converges as $m\to+\infty$,
for every function $f\in\mathcal{C}\big(\partial\mathbb{D}\big)$,
hence there exists a limit function, denoted by $\Lambda f$, such that
\begin{equation}\label{mu-s3}
\lim_{m\to+\infty}\int_{\partial\mathbb{D}}f(z)\,{\rm d}\mu_{s_m}=\Lambda f\; ,
\quad \forall f\in\mathcal{C}\big(\partial\mathbb{D}\big)\;.
\end{equation}
Clearly, this defines a linear functional
$\Lambda:\mathcal{C}\big(\partial\mathbb{D}\big)\rightarrow\mathbb{C}$.
Since $\frac{{\rm d}\mu_s}{{\rm d}z}\geq0$, we obtain
\begin{equation}\label{mu-s4}
\Lambda f\geq0 \quad\mbox{\rm whenever}\quad f\geq0
\qquad\big(\forall f\in\mathcal{C}\big(\partial\mathbb{D}\big)\big)\; ,
\end{equation}
hence $\Lambda$ is a positive linear functional
in $\mathcal{C}\big(\partial\mathbb{D}\big)$. Thus, since
$\partial\mathbb{D}$ is a compact set, it follows from the
Riesz-Kakutani Theorem that there exists a
probability measure $\mu$ on $\partial\mathbb{D}$ such that
\begin{equation}\label{mu-s5}
\Lambda f=\int_{\partial\mathbb{D}}f(z)\,{\rm d}\mu\; ,
\quad \forall f\in\mathcal{C}\big(\partial\mathbb{D}\big)\;.
\end{equation}
Next, using successively (\ref{mu-s5}), (\ref{mu-s3}), and (\ref{mu-s2}),
we deduce
$$
\int_{\partial\mathbb{D}}z^{-k}\,{\rm d}\mu=\Lambda(z^{-k})
=\lim_{m\to+\infty}\int_{\partial\mathbb{D}}z^{-k}\,{\rm d}\mu_{s_m}=c_{-k}\; ,\quad
\forall k\in\mathbb{Z}\;.
$$
This proves (\ref{cn-int1}), i.e., the existence part of the theorem.
\smallskip

(ii)
Conversely, suppose that $(c_n)_{n\in\mathbb{Z}}$ is a sequence of complex numbers
defined by (\ref{cn-int1}) for some finite non-negative measure on $\partial\mathbb{D}$.
Then, for every $N\in\mathbb{N}_0$ and any sequence $(a_n)_{n\in\mathbb{N}_0}\subset\mathbb{C}$,
$$
\begin{array}{rcl}
\displaystyle\sum_{n,m=0}^Nc_{n-m}a_n\overline{a}_m
&=& \displaystyle\sum_{n,m=0}^Na_n\overline{a}_m\int_{\partial\mathbb{D}}z^{n-m}\,{\rm d}\mu
\,=\,\int_{\partial\mathbb{D}}\Big|\sum_{n=0}^Na_nz^n\Big|^2\,{\rm d}\mu\geq0\; ,
\end{array}
$$
hence $(c_n)_{n\in\mathbb{Z}}$ is a positive-definite sequence in $\mathbb{C}$.
\smallskip

(iii) Finally, we prove the uniqueness of $\mu$.
Let $\mu$ and $\nu$ be two finite non-negative measures on $\partial\mathbb{D}$
such that (\ref{cn-int1}) holds for $\mu$ and $\nu$, i.e.,
$$
\int_{\partial\mathbb{D}}z^{n}\,{\rm d}\mu=c_n
=\int_{\partial\mathbb{D}}z^{n}\,{\rm d}\nu\;,\quad\forall n\in\mathbb{Z}\;.
$$
Then $\int_{\partial\mathbb{D}}p(z)\,{\rm d}\mu
=\int_{\partial\mathbb{D}}p(z)\,{\rm d}\nu$
for every $p\in\langle \{z^n\}_{n\in\mathbb{Z}}\rangle$, i.e.,
$p(z)$ a finite linear combination of positive or negative powers of $z$.
Therefore, since the set $\langle \{z^n\}_{n\in\mathbb{Z}}\rangle$
is dense in $\mathcal{C}\big(\partial\mathbb{D}\big)$, we obtain
$$
\int_{\partial\mathbb{D}}f(z)\,{\rm d}\mu
=\int_{\partial\mathbb{D}}f(z)\,{\rm d}\nu\; ,\quad
\forall f\in\mathcal{C}\big(\partial\mathbb{D}\big)\;.
$$
This implies $\mu=\nu$.
\qed

\section{Spectral Theorem for unitary operators}


\begin{snugshade}
\begin{theorem}\label{Spectral-Thm}
Let $U$ be a unitary operator on a separable Hilbert space $\mathcal{H}$.
Let $x$ be a cyclic vector for $U$ in $\mathcal{H}$.
Then, there exists a unique measure $\mu$ on the unit circle $\mathbb{D}$
---or, equivalently, a measure on the interval $[0,2\pi]$--- such that
\begin{equation}\label{intUv}
\langle U^nx,x\rangle=\int_{\partial\mathbb{D}}z^n\,{\rm d}\mu(z)
:=\int_0^{2\pi}e^{in\theta}\,{\rm d}\mu(\theta)\; ,\quad\forall n\in\mathbb{Z}\,.
\end{equation}
\end{theorem}
\end{snugshade}

{\it Proof.}
The result follows immediately from (Herglotz) Theorem \ref{Herglotz-Thm},
noticing that the sequence $(c_n)_{n\in\mathbb{Z}}$ defined by
$$
c_n:=\langle U^nx,x\rangle\; ,\quad n\in\mathbb{Z}\; ,
$$
is a positive-definite sequence in $\mathbb{C}$.
Indeed, being $U$ a unitary operator, then $UU^*=U^*U=I$ and $U^{-1}=U^*$,
hence we deduce $c_{n-m}=\langle U^{n-m}x,x\rangle=\langle U^{n}x,U^{m}x\rangle$
for every $n,m\in\mathbb{Z}$. Therefore, for every $N\in\mathbb{N}_0$
and every sequence $(a_n)_{n\in\mathbb{N}_0}\subset\mathbb{C}$, we may write
$$
\sum_{n,m=0}^Nc_{n-m}a_n\overline{a}_m
=\big\langle\sum_{n=0}^Na_nU^nx,\sum_{m=0}^Na_mU^mx\big\rangle
=\Big\|\sum_{n=0}^Na_nU^n\Big\|^2\geq0\; ,
$$
and so $(c_n)_{n\in\mathbb{Z}}$ is a positive-definite sequence in $\mathbb{C}$.
\qed


\section{Remarks and historical notes}




\section*{Exercises}
%\bigskip

%\noindent
\begin{enumerate}[label=\emph{\bf \arabic*.},leftmargin=*]
\item Ex 1
\medskip

%\item
%Sejam $X$ um e.v. real, $p:X\rightarrow\mathbb{R}$ uma funcional sublinear e
%$K:=\{\,x\in X\,|\, p(x)<1\,\}\,$. Mostre que: % $K$ satisfaz as propriedades seguintes:
%\begin{enumerate}
%\item $K$ \'e convexo;
%\item $0$ \'e um ponto interior de $K$ (no sentido da Defini\c c\~ao \ref{def-pontoInt});%(no sentido alg\'ebrico).
%\item $p$ \'e a funcional de Minkowski do conjunto $K$.
%\end{enumerate}
%\medskip

\item
Ex 3
\end{enumerate}
\bigskip

%\medskip

\section*{Bibliography}
%\medskip

{\small
\begin{enumerate}[label=\emph{\rm [\arabic*]},leftmargin=*]
\item\label{Parry2004} W. Parry, {\sl Topics in Ergodic Theory},
          Cambridge University Press (1981) [paperback edition: 2004].
%\item\label{ReedSimon1972i} M. Reed and B. Simon, {\sl Methods of Modern Mathematical Physics I: Functional Analysis},
%Academic Press (1972).
%\item\label{Szegoo1975i} G. Szeg\"o, {\sl Orthogonal Polynomials}, AMS Colloq. Publ. {\bf 230} (1975), 4th ed.
\end{enumerate}
}



==> opsf_t12_2016-17.tex <==


\chapter{Orthogonal polynomials on the unit circle}

\pagestyle{myheadings}\markright{Orthogonal polynomials on the unit circle}
\pagestyle{myheadings}\markleft{J. Petronilho}

One of the most important 


\section{Positive-definite sequences}


\begin{snugshade}
\begin{definition}
A sequence of numbers $(c_n)_{n\in\mathbb{Z}}\subset\mathbb{C}$
is called {\sl positive-definite} if
\begin{equation}%\label{posit-seq1}
\sum_{n,m=0}^Nc_{n-m}a_n\overline{a}_m\geq0\; ,
\quad\forall(a_n)_{n\in\mathbb{N}_0}\subset\mathbb{C}\;,\;\forall N\in\mathbb{N}_0\; .
\end{equation}
\end{definition}
\end{snugshade}
\noindent
The following proposition lists some basic properties of positive-definite sequences.

\begin{snugshade}
\begin{proposition}%\label{prop-posit-seq1}
Let $(c_n)_{n\in\mathbb{Z}}$ be a positive-definite sequence. % in $\mathbb{C}$.
Then: \smallskip %the following properties hold:
$$
\begin{array}{rl}
\mbox{\rm (i)} & c_0\big(|a|^2+|b|^2\big)+c_n\overline{a}b+c_{-n}a\overline{b}\geq0\;,\;
\forall n\in\mathbb{Z}\; ,\; \forall a,b\in\mathbb{C}\; ; \\ [0.6em]
\mbox{\rm (ii)} & c_{-n}=\overline{c_n}\; ,\; \forall n\in\mathbb{Z}\; ;\\ [0.6em]
\mbox{\rm (iii)} & |c_{n}|\leq c_0\; ,\; \forall n\in\mathbb{Z}\; .
\end{array}
$$
\end{proposition}
\end{snugshade}

{\it Proof.}


\qed

\begin{remark}%\label{c0=1} \em
%We emphasize that
Property (iii) in 
\end{remark}


\section{Szeg\"o Theorem}

As usual, 


\section{Remarks and historical notes}




\section*{Exercises}
%\bigskip

%\noindent
\begin{enumerate}[label=\emph{\bf \arabic*.},leftmargin=*]
\item Ex 1
\medskip

%\item
%Sejam $X$ um e.v. real, $p:X\rightarrow\mathbb{R}$ uma funcional sublinear e
%$K:=\{\,x\in X\,|\, p(x)<1\,\}\,$. Mostre que: % $K$ satisfaz as propriedades seguintes:
%\begin{enumerate}
%\item $K$ \'e convexo;
%\item $0$ \'e um ponto interior de $K$ (no sentido da Defini\c c\~ao \ref{def-pontoInt});%(no sentido alg\'ebrico).
%\item $p$ \'e a funcional de Minkowski do conjunto $K$.
%\end{enumerate}
%\medskip

\item
Ex 3
\end{enumerate}
\bigskip

%\medskip

\section*{Bibliography}
%\medskip

{\small
\begin{enumerate}[label=\emph{\rm [\arabic*]},leftmargin=*]
\item\label{Parry2004} W. Parry, {\sl Topics in Ergodic Theory},
          Cambridge University Press (1981) [paperback edition: 2004].
%\item\label{ReedSimon1972i} M. Reed and B. Simon, {\sl Methods of Modern Mathematical Physics I: Functional Analysis},
%Academic Press (1972).
%\item\label{Szegoo1975i} G. Szeg\"o, {\sl Orthogonal Polynomials}, AMS Colloq. Publ. {\bf 230} (1975), 4th ed.
\end{enumerate}
}



==> opsf_t13_2016-17.tex <==


\chapter{Hypergeometric functions}

\pagestyle{myheadings}\markright{Hypergeometric functions}
\pagestyle{myheadings}\markleft{J. Petronilho}

One of the most important


\section{Positive-definite sequences}


\begin{snugshade}
\begin{definition}
A sequence of numbers $(c_n)_{n\in\mathbb{Z}}\subset\mathbb{C}$
is called {\sl positive-definite} if
\begin{equation}%\label{posit-seq1}
\sum_{n,m=0}^Nc_{n-m}a_n\overline{a}_m\geq0\; ,
\quad\forall(a_n)_{n\in\mathbb{N}_0}\subset\mathbb{C}\;,\;\forall N\in\mathbb{N}_0\; .
\end{equation}
\end{definition}
\end{snugshade}
\noindent
The following proposition lists some basic properties of positive-definite sequences.

\begin{snugshade}
\begin{proposition}%\label{prop-posit-seq1}
Let $(c_n)_{n\in\mathbb{Z}}$ be a positive-definite sequence. % in $\mathbb{C}$.
Then: \smallskip %the following properties hold:
$$
\begin{array}{rl}
\mbox{\rm (i)} & c_0\big(|a|^2+|b|^2\big)+c_n\overline{a}b+c_{-n}a\overline{b}\geq0\;,\;
\forall n\in\mathbb{Z}\; ,\; \forall a,b\in\mathbb{C}\; ; \\ [0.6em]
\mbox{\rm (ii)} & c_{-n}=\overline{c_n}\; ,\; \forall n\in\mathbb{Z}\; ;\\ [0.6em]
\mbox{\rm (iii)} & |c_{n}|\leq c_0\; ,\; \forall n\in\mathbb{Z}\; .
\end{array}
$$
\end{proposition}
\end{snugshade}

{\it Proof.}


\qed

\begin{remark}%\label{c0=1} \em
%We emphasize that
Property (iii) in
\end{remark}


\section{Szeg\"o Theorem}

As usual,


\section{Remarks and historical notes}




\section*{Exercises}
%\bigskip

%\noindent
\begin{enumerate}[label=\emph{\bf \arabic*.},leftmargin=*]
\item Ex 1
\medskip

%\item
%Sejam $X$ um e.v. real, $p:X\rightarrow\mathbb{R}$ uma funcional sublinear e
%$K:=\{\,x\in X\,|\, p(x)<1\,\}\,$. Mostre que: % $K$ satisfaz as propriedades seguintes:
%\begin{enumerate}
%\item $K$ \'e convexo;
%\item $0$ \'e um ponto interior de $K$ (no sentido da Defini\c c\~ao \ref{def-pontoInt});%(no sentido alg\'ebrico).
%\item $p$ \'e a funcional de Minkowski do conjunto $K$.
%\end{enumerate}
%\medskip

\item
Ex 3
\end{enumerate}
\bigskip

%\medskip

\section*{Bibliography}
%\medskip

{\small
\begin{enumerate}[label=\emph{\rm [\arabic*]},leftmargin=*]
\item\label{Parry2004} W. Parry, {\sl Topics in Ergodic Theory},
          Cambridge University Press (1981) [paperback edition: 2004].
%\item\label{ReedSimon1972i} M. Reed and B. Simon, {\sl Methods of Modern Mathematical Physics I: Functional Analysis},
%Academic Press (1972).
%\item\label{Szegoo1975i} G. Szeg\"o, {\sl Orthogonal Polynomials}, AMS Colloq. Publ. {\bf 230} (1975), 4th ed.
\end{enumerate}
}



==> opsf_t15_2016-17.tex <==


\chapter{Orthogonal polynomials on several variables}

\pagestyle{myheadings}\markright{Orthogonal polynomials on several variables}
\pagestyle{myheadings}\markleft{J. Petronilho}



\section{Section 1}






\section{Remarks and historical notes}




\section*{Exercises}
%\bigskip

%\noindent
\begin{enumerate}[label=\emph{\bf \arabic*.},leftmargin=*]
\item Ex 1
\medskip

%\item
%Sejam $X$ um e.v. real, $p:X\rightarrow\mathbb{R}$ uma funcional sublinear e
%$K:=\{\,x\in X\,|\, p(x)<1\,\}\,$. Mostre que: % $K$ satisfaz as propriedades seguintes:
%\begin{enumerate}
%\item $K$ \'e convexo;
%\item $0$ \'e um ponto interior de $K$ (no sentido da Defini\c c\~ao \ref{def-pontoInt});%(no sentido alg\'ebrico).
%\item $p$ \'e a funcional de Minkowski do conjunto $K$.
%\end{enumerate}
%\medskip

\item
Ex 3
\end{enumerate}
\bigskip

%\medskip

\section*{Bibliography}
%\medskip

{\small
\begin{enumerate}[label=\emph{\rm [\arabic*]},leftmargin=*]
\item\label{Rudin1986} W. Rudin, {\sl Real and Complex Analysis},
          McGraw-Hill (1986) [paperback edition: 2004].
%\item\label{ReedSimon1972i} M. Reed and B. Simon, {\sl Methods of Modern Mathematical Physics I: Functional Analysis},
%Academic Press (1972).
%\item\label{Szegoo1975i} G. Szeg\"o, {\sl Orthogonal Polynomials}, AMS Colloq. Publ. {\bf 230} (1975), 4th ed.
\end{enumerate}
}



==> opsf_tOPRLBorelmeasures6_2015-16.tex <==

%\chapter{Orthogonality with respect to positive functionals}
%\chapter{Orthogonality with respect to a positive Borel mesure}

\chapter{OPRL with respect to positive Borel measures}

%\chapter{Topological preliminaries}
\pagestyle{myheadings}\markright{OPRL}
\pagestyle{myheadings}\markleft{J. Petronilho}

%\chapter{Teorema de Hahn-Banach num e.v.$\,-\,$forma anal\'\i tica}
%\chapter{Teoremas de Hahn-Banach. Separa\c c\~ao de conjuntos convexos}
%\pagestyle{myheadings}\markright{Teorema de Hahn-Banach num e.v.$\,-\,$forma anal\'\i tica}

The Riesz-Markov-Kakutani representation theorem establishes
a duality relation between


Before stating the Riesz-Markov-Kakutani theorem we will review some useful results,
namely the famous Urysohn's Lemma and some properties involving the concept
of partition of unity of a compact set subordinate to an open cover.


\section{OPRL}

\section{Jacobi operators}



\section{Stieltjes-Favard Theorem}

\begin{snugshade}
\begin{theorem}[Stieltjes-Favard]\label{Favard}
Let $a\equiv\big(a_n\big)_{n\in\mathbb{N}}\subset\mathbb{R}_+$ and $b\equiv\big(b_n\big)_{n\in\mathbb{N}_0}\subset\mathbb{R}$, and let ${\bf J}\equiv {\bf J}(a,b)$ be the associated Jacobi operator. Assume that ${\bf J}$ is bounded on $\ell^2\equiv\ell^2(\mathbb{C})$, i.e.,
$$
{\bf J}\in\mathcal{B}\big(\ell^2\big)\; .
$$
Then the following holds:
\begin{enumerate}
\item[{\rm (i)}] ${\bf J}$ is self-adjoint on $\ell^2$;
\item[{\rm (ii)}] $e_0$ is a cyclic vector for ${\bf J}$, and the set of Jacobi parameters for the
corresponding spectral measure $\mu$ is $\{a,b\}$;
\item[{\rm (iii)}] if $\nu$ is a compactly supported nontrivial probability measure on $\mathbb{R}$ with Jacobi parameters $\{a,b\}$, then $\nu=\mu$.
\item[{\rm (iv)}] The mapping
$$
\varphi:\mathfrak{M}_0\to\mathbb{R}_+^\infty\times\mathbb{R}^\infty\quad \big(\;\mu\mapsto\{a,b\}\;\big)
$$
is a bijection between the set of compactly supported nontrivial probability measures on $\mathbb{R}$ and the set of sequences $\{a,b\}$ with $a\subset(0,+\infty)$ and $b\subset\mathbb{R}$.
\end{enumerate}
\end{theorem}
\end{snugshade}

{\it Proof.}

\qed


\section{Zeros of OPRL}

\section{Examples}

\begin{snugshade}
\begin{definition}\label{defnova}
Let $X$ be a Hausdorff space and
$\Lambda:\mathcal{C}_0(X)\to\mathbb{K}$ linear.
$\Lambda$ is called a {\sl positive linear functional} if
$\Lambda f\geq0$ for every function $f\in\mathcal{C}_0(X)$ such that $f\geq0$; i.e.,
$$
f(X)\subset[0,+\infty[\quad\Rightarrow\quad \Lambda f\geq0\;,\qquad\forall f\in\mathcal{C}_0(X)\;.
$$
\end{definition}
\end{snugshade}


\section{Remarks and historical notes}




\section*{Exercises}
%\bigskip

%\noindent
\begin{enumerate}[label=\emph{\bf \arabic*.},leftmargin=*]
\item Ex 1
\medskip

%\item
%Sejam $X$ um e.v. real, $p:X\rightarrow\mathbb{R}$ uma funcional sublinear e
%$K:=\{\,x\in X\,|\, p(x)<1\,\}\,$. Mostre que: % $K$ satisfaz as propriedades seguintes:
%\begin{enumerate}
%\item $K$ \'e convexo;
%\item $0$ \'e um ponto interior de $K$ (no sentido da Defini\c c\~ao \ref{def-pontoInt});%(no sentido alg\'ebrico).
%\item $p$ \'e a funcional de Minkowski do conjunto $K$.
%\end{enumerate}
%\medskip

\item
Ex 3
\end{enumerate}
\bigskip

%\medskip

\section*{Bibliography}
%\medskip

{\small
\begin{enumerate}[label=\emph{\rm [\arabic*]},leftmargin=*]
\item\label{Rudin1986} W. Rudin, {\sl Real and Complex Analysis},
          McGraw-Hill (1986) [paperback edition: 2004].
%\item\label{ReedSimon1972i} M. Reed and B. Simon, {\sl Methods of Modern Mathematical Physics I: Functional Analysis},
%Academic Press (1972).
%\item\label{Szegoo1975i} G. Szeg\"o, {\sl Orthogonal Polynomials}, AMS Colloq. Publ. {\bf 230} (1975), 4th ed.
\end{enumerate}
}



==> opsf_tRiezMarkovKakutani_2015-16.tex <==

%\setcounter{page}{1}

%\chapter{Preliminaries on Functional Analysis}

%\chapter{A crash course on locally convex spaces}

\chapter{The Riesz-Markov-Kakutani Theorem}

%\chapter{Topological preliminaries}
\pagestyle{myheadings}\markright{The Riesz-Markov-Kakutani Theorem}
\pagestyle{myheadings}\markleft{J. Petronilho}

%\chapter{Teorema de Hahn-Banach num e.v.$\,-\,$forma anal\'\i tica}
%\chapter{Teoremas de Hahn-Banach. Separa\c c\~ao de conjuntos convexos}
%\pagestyle{myheadings}\markright{Teorema de Hahn-Banach num e.v.$\,-\,$forma anal\'\i tica}

The Riesz-Markov-Kakutani representation theorem establishes
a duality relation between


Before stating the Riesz-Markov-Kakutani theorem we will review some useful results,
namely the famous Urysohn's Lemma and some properties involving the concept
of partition of unity of a compact set subordinate to an open cover.


\section{Topological Preliminaries}

Here

\subsection{Urysohn's Lemma}

Here


\begin{snugshade}
\begin{theorem}[Urysohn's Lemma]\label{Urysohn1}
Suppose that $X$ is a locally compact Hausdorff space, $V$ is open in $X$, $K\subset V$, and $K$ is compact. Then
\begin{equation}\label{KfV}
\exists f\in\mathcal{C}_0(X)\; :\quad K \prec f \prec V\; .
\end{equation}
\end{theorem}
\end{snugshade}

{\it Proof.}

\qed




\section{Partitions of unity}

Here


\begin{snugshade}
\begin{theorem}[existence of partitions of unity]\label{ThmPUnity1}
Suppose that $X$ is a locally compact Hausdorff space, $V_1,\ldots,V_n$ are open subsets of $X$, $K$ is compact, and
$$
K\subseteq V_1\cup\cdots\cup V_n\;.
$$
Then, there exists functions $h_1,\ldots,h_n$ such that
\begin{equation}\label{PUnity1}
h_i\prec V_i\quad(1,\cdots,n)\; ,\quad h_1(x)+\cdots+h_n(x)=1\quad(x\in K)\; .
\end{equation}
\end{theorem}
\end{snugshade}

{\it Proof.}

\qed

\begin{snugshade}
\begin{definition}\label{defPUnity}
Under the conditions of Theorem \ref{ThmPUnity1}, the collection of functions
$\{h_1,\ldots,h_n\}$ is called a {\sl partition of unity on $K$},
subordinate to the cover $\{V_1,\ldots,V_n\}$.
\end{definition}
\end{snugshade}



\section{Riesz-Markov-Kakutani Theorem}

\begin{snugshade}
\begin{definition}\label{Lamb}
Let $X$ be a Hausdorff space and
$\Lambda:\mathcal{C}_0(X)\to\mathbb{K}$ linear.
$\Lambda$ is called a {\sl positive linear functional} if
$\Lambda f\geq0$ for every function $f\in\mathcal{C}_0(X)$ such that $f\geq0$; i.e.,
$$
\forall f\in\mathcal{C}_0(X)\;,\quad
f(X)\subseteq[0,+\infty[\quad\Rightarrow\quad \Lambda f\geq0\;.
$$
\end{definition}
\end{snugshade}

Here

\begin{snugshade}
\begin{theorem}[Riesz-Markov-Kakutani]\label{Riesz-Markov-Kakutani-Thm}
Let $X$ be a locally compact Hausdorff space, and let $\Lambda$ be a
positive linear functional on $\mathcal{C}_0(X)$.
Then, there exists a $\sigma-$algebra $\mathcal{A}$ in $X$ containing all Borel sets in $X$,
and there exists a unique positive measure $\mu$ on $\mathcal{A}$ which represents $\Lambda$
in the sense that
\begin{equation}\label{repres-Lambda}
\Lambda f=\int_{X}f\,{\rm d}\mu\; ,\quad\forall f\in\mathcal{C}_0(X)\;,
\end{equation}
and which has the following additional properties:
\begin{enumerate}
\item[{\rm (i)}] $\mu(K)<\infty$ for all compact set $K\subset X$;
\item[{\rm (ii)}] for every $E\in\mathcal{A}$,
$$
\mu(E)=\inf\big\{ \mu(V)\,|\,E\subset V\;,\; \mbox{\rm $V$ open}\big\}\; ;
$$
\item[{\rm (iii)}] the relation
$$
\mu(E)=\sup\big\{ \mu(K)\,|\,K\subset E\;,\; \mbox{\rm $K$ compact}\big\}
$$
holds for every open set $E$, and for every $E\in\mathcal{A}$ with $\mu(E)<\infty$;
\item[{\rm (iv)}] if $E\in\mathcal{A}$, $A\subset E$, and $\mu(E)=0$, then $A\in\mathcal{A}$.
\end{enumerate}
\end{theorem}
\end{snugshade}

{\it Proof.}
We begin by constructing $\mu$ and $\mathcal{A}$.
For every open set $V$ in $X$, define
\begin{equation}\label{Rudin1}
\mu(V):=\sup\big\{ \Lambda f\,|\, f \prec V \big\}\, ,
\end{equation}
and then, for every $E\subseteq X$, define
\begin{equation}\label{Rudin2}
\mu(E):=\inf\big\{ \mu(V)\,|\, E\subseteq V\;,\; \mbox{\rm $V$ open}\, \big\}\, .
\end{equation}
Notice that definitions (\ref{Rudin1}) and (\ref{Rudin2}) are consistent,
since (\ref{Rudin1}) clearly implies
$$
\mbox{\rm $V_1$, $V_2$ open sets in $X$,}\quad
V_1\subseteq V_2\quad\Rightarrow\quad \mu(V_1)\leq\mu(V_2)\; .
$$
Notice also that, although we have defined $\mu(E)$ for every $E\subseteq X$,
the countable additivity of $\mu$ will be proved only on a
certain $\sigma-$algebra $\mathcal{A}$ in $X$ (containing all Borel sets in $X$).
Let
\begin{equation}\label{Rudin3}
\mathcal{A}_F:=\Big\{ E\subseteq X\,|\, \mu(E)<\infty\; \wedge\;
\mu(E)=\sup\big\{ \mu(K)\,|\, K\subseteq E\;,\; \mbox{\rm $K$ compact}\, \big\}\, \Big\}\;,
\end{equation}
and, finally, set
$$
\mathcal{A}:=\big\{\, E\subseteq X\,|\, E\cap K\in\mathcal{A}_F\;,\;
\forall\;\mbox{\rm $K$ compact}\, \big\}\,.
$$
We will prove that $\mu$ and $\mathcal{A}$ have all the required properties.
We begin by noticing that $\mu$ is monotone, i.e., $\mu(A)\leq\mu(B)$ if $A\subseteq B$,
and that $\mu(E)=0$ implies $E\in\mathcal{A}_F$ and $E\in\mathcal{A}$.
Thus (iv) holds, and so does (ii), by definition.

Since the proof of the remaining assertions is rather long,
it will be convenient to divide it into several steps.
\smallskip

{\bf Step 1.}
{\it If $E_1,E_2,E_3,\ldots$ are arbitrary subsets of $X$, then}
\begin{equation}\label{Rudin4}
\mu\Big(\bigcup_{k=1}^\infty E_k\Big)\leq\sum_{k=1}^\infty \mu(E_k)\; .
\end{equation}
{\it Proof.}
We first show that, for every open sets $V_1$ and $V_2$,
\begin{equation}\label{Rudin5}
\mu(V_1\cup V_2)\leq\mu(V_1)+\mu(V_2)\; .
\end{equation}
Choose arbitrarily $g\prec V_1\cup V_2$.
By Theorem \ref{ThmPUnity1}, there are functions $h_1$ and $h_2$ such that
$$
h_1\prec V_1\;,\quad h_2\prec V_2\;,\quad h_1(x)+h_2(x)=1\; ,\; \forall x\in\mbox{\rm spt}\,g\;.
$$
Hence, clearly, $h_1g\prec V_1$, $h_2g\prec V_2$, and $g=h_1g+h_2g$, and so,
by the linearity of $\Lambda$ and taking into account (\ref{Rudin1}),
$$%\begin{equation}\label{Rudin6}
\Lambda g=\Lambda(h_1g)+\Lambda(h_2g)\leq
\sup\big\{ \Lambda f\,|\, f \prec V_1\big\}+\sup\big\{ \Lambda f\,|\, f \prec V_2\big\}
\leq\mu(V_1)+\mu(V_2)\; .
$$%\end{equation}
We may conclude that $\;g\prec V_1\cup V_2\;\Rightarrow\;\Lambda g\leq\mu(V_1)+\mu(V_2)\,$,
hence, using again (\ref{Rudin1}),
%$$
%g\prec V_1\cup V_2\quad\Rightarrow\quad\Lambda g\leq\mu(V_1)+\mu(V_2)\; .
%$$
%Therefore, using again (\ref{Rudin1}),
$$
\mu(V_1\cup V_2)=\sup\big\{ \Lambda g\,|\, g \prec V_1\cup V_2 \big\}\leq\mu(V_1)+\mu(V_2)\, ,
$$
and so (\ref{Rudin5}) is proved.

Now, if $\mu(E_k)=\infty$ for some $k\in\mathbb{N}$, then (\ref{Rudin4}) holds trivially.
Suppose therefore that $\mu(E_k)<\infty$ for every $k\in\mathbb{N}$. Choose $\epsilon>0$.
By (\ref{Rudin2}) and the definition of infimum, there are open sets $V_1,V_2,\ldots$
such that $E_k\subseteq V_k$ for every $k\in\mathbb{N}$ and
$$
\mu(V_k)\leq\mu(E_k)+\frac{\epsilon}{2^k}\;,\quad k=1,2\cdots\; .
$$
Set $V:=\bigcup_{k=1}^\infty V_k$ (which is an open set) and choose arbitrarily $f\prec V$.
Since $\mbox{\rm spt}\,f\subset V$ and $\mbox{\rm spt}\,f$ is compact,
then $\mbox{\rm spt}\,f$ may be covered by a finite number of open sets $V_k$'s,
so there exists $n\in\mathbb{N}$ such that $f\prec V_1\cup\cdots\cup V_n$. Therefore, by (\ref{Rudin1}),
\begin{equation}\label{Rudin5a}
\Lambda f\leq\mu(V_1\cup\cdots\cup V_n)\leq\mu(V_1)+\cdots+\mu(V_n)\leq\sum_{k=1}^\infty\mu(V_k)+\epsilon\; ,
\end{equation}
the second inequality being justified by applying induction to (\ref{Rudin5}).
Since $V$ is open and (\ref{Rudin5a}) holds for every $f\prec V$, then, using again (\ref{Rudin1}),
$$
\mu(V)\leq\sum_{k=1}^\infty\mu(V_k)+\epsilon\; ,
$$
and so, since $\bigcup_{k=1}^\infty E_k\subseteq\bigcup_{k=1}^\infty V_k=:V$,
it follows from (\ref{Rudin2}) that
$$
\mu\Big(\bigcup_{k=1}^\infty E_k\Big)\leq\mu(V)\leq\sum_{k=1}^\infty \mu(E_k)+\epsilon\; .
$$
This proves (\ref{Rudin4}), since $\epsilon$ was arbitrary.
\medskip

{\bf Step 2.} {\it The following holds:}
\begin{equation}\label{Rudin7}
\mbox{\it $K$ compact}\quad\Rightarrow\quad
K\in\mathcal{A}_F\quad\wedge\quad \mu(K)=\inf\{\Lambda f\,|\, K\prec f\}\; .
\end{equation}
{\it Proof.}
Let $K$ be any compact subset of $X$.
For $f$ such that $K\prec f$ and $0<\alpha<1$, set
$V_\alpha:=\{x\in\, X|\,f(x)>\alpha\}=f^{-1}\big((\alpha,+\infty)\big)$.
%Since $V_\alpha=f^{-1}\big((\alpha,+\infty)\big)$ and
Since $f$ is continuous, %we see that
$V_\alpha$ is open.
Also, $K\subset V_\alpha$ (because, being $K\prec f$, we have $x\in K\Rightarrow f(x)=1>\alpha\Rightarrow x\in V_\alpha$)
and $\alpha g\leq f$ whenever $g\prec V_\alpha$ (since this implies $0\leq g\leq 1$, so
$x\in V_\alpha\Rightarrow f(x)>\alpha\geq\alpha g(x)$). Hence, using (\ref{Rudin2}) and (\ref{Rudin1}),
$$
\mu(K)\leq\mu(V_\alpha)=\sup\big\{ \Lambda g\,|\, g \prec V_\alpha\big\}\leq\alpha^{-1}\,\Lambda f\;.
$$
Letting $\alpha\to1$, we conclude that
\begin{equation}\label{Rudin8}
\mbox{\it $K$ compact}\;\;\wedge\;\;K\prec f\quad\Rightarrow\quad\mu(K)\leq\Lambda f\;.
\end{equation}
%\begin{equation}\label{Rudin8}
%\mu(K)\leq\Lambda f\;.
%\end{equation}
Thus, for any compact $K$, we have $\mu(K)<\infty$, and so $K\in\mathcal{A}_F$
(since, being compact, $K$ clearly satisfies the second condition in the definition of $\mathcal{A}_F$).
It remains to prove that $\mu(K)=\inf\{\Lambda f\,|\, K\prec f\}$.
Let $\epsilon>0$. By (\ref{Rudin2}), there exists an open set $V$
such that $V\supset K$ and $\mu(V)<\mu(K)+\epsilon$.
By Urysohn's Lemma (Theorem \ref{Urysohn1}),
$K\prec f\prec V$ for some $f\in\mathcal{C}_0(X)$. Thus, by (\ref{Rudin1}),
$$
\Lambda f\leq\mu(V)<\mu(K)+\epsilon\; ,
$$
which, combined with (\ref{Rudin8}), gives $\mu(K)=\inf\{\Lambda f\,|\, K\prec f\}$.
Hence (\ref{Rudin7}) holds.
\medskip

{\bf Step 3.} {\it Every open set $V$ satisfies the second condition in the definition of $\mathcal{A}_F$:
\begin{equation}\label{Rudin3a}
\mu(V)=\sup\{\mu(K)\,|\, K\subset V\;,\;\mbox{\rm $K$ compact}\}\;;
\end{equation}
hence $\mathcal{A}_F$ contains every open set $V$ with $\mu(V)<\infty$.}
\smallskip

{\it Proof.}
By definition of supremum, we need to show that $\mu(V)\geq\mu(K)$
for every compact $K\subset V$, and that, for any $\epsilon>0$,
there exists a compact $K\subset V$ such that $\mu(V)<\mu(K)+\epsilon$.
Indeed, if $K\subset V$, (\ref{Rudin2}) gives immediately $\mu(V)\geq\mu(K)$.
On the other hand, let $\epsilon>0$.
%Since (\ref{Rudin3a}) is trivial if $\mu(V)=0$, we may assume that $\mu(V)>0$.
Set $\alpha:=\mu(V)-\epsilon$. Then $\alpha<\mu(V)$,
hence, by (\ref{Rudin1}), there exists an $f\prec V$ with $\alpha<\Lambda f$.
If $W$ is any open set which contains $K:=\mbox{\rm spt}\,f$, then $f\prec W$,
hence, by (\ref{Rudin1}), $\Lambda f\leq\mu(W)$.
Thus, $\Lambda f\leq\inf\{\mu(W)\,|\,W\supset K\,,\,\mbox{\rm $W$ open}\}=\mu(K)$,
by (\ref{Rudin2}), and so $\alpha<\mu(K)$.
Moreover, $K\subset V$ (since $f\prec V$ and $K=\mbox{\rm spt}\,f$).
We have shown that, for every $\epsilon>0$ we may find a compact set $K\subset V$
such that $\mu(V)<\mu(K)+\epsilon$, so that (\ref{Rudin3a}) holds.
\medskip

{\bf Step 4.}
{\it Suppose that $E=\bigcup_{k=1}^\infty E_k$, where $E_1,E_2,E_3,\ldots$ are pairwise disjoint
members of $\mathcal{A}_F$. Then
\begin{equation}\label{Rudin9}
\mu(E)=\sum_{k=1}^\infty\mu(E_k)\;.
\end{equation}
If, in addition, $\mu(E)<\infty$, then also $E\in\mathcal{A}_F$.}
\smallskip

{\it Proof.}
We first show that if $K_1$ and $K_2$ are disjoint compact sets, then
\begin{equation}\label{Rudin10}
\mu(K_1\cup K_2)=\mu(K_1)+\mu(K_2)\;.
\end{equation}
Indeed, by Step 1, we have $\mu(K_1\cup K_2)\leq\mu(K_1)+\mu(K_2)$.
To prove that the reverse inequality also holds, choose arbitrarily $\epsilon>0$.
By Urysohn's Lemma, there exists $f\in\mathcal{C}_0(X)$
such that $f=1$ on $K_1$, $f=0$ on $K_2$, and $0\leq f\leq1$.
Since $K_1\cup K_2$ is compact, by Step 2 and the definition of infimum,
there exists $g\in\mathcal{C}_0(X)$ such that
$$
K_1\cup K_2\prec g\; ,\quad \Lambda g<\mu(K_1\cup K_2)+\epsilon\;.
$$
Note that, clearly, $K_1\prec fg$ and $K_2\prec (1-f)g$.
Hence, since $\Lambda$ is linear, it follows from (\ref{Rudin8}) that
$$
\mu(K_1)+\mu(K_2)\leq \Lambda(fg)+\Lambda\big((1-f)g\big)
=\Lambda g<\mu(K_1\cup K_2)+\epsilon\;.
$$
Letting $\epsilon\to0$ we obtain $\mu(K_1)+\mu(K_2)\leq\mu(K_1\cup K_2)$,
and so (\ref{Rudin10}) is proved.

Next, if $\mu(E)=\infty$, then (\ref{Rudin9}) follows by Step 1.
Assume therefore that $\mu(E)<\infty$. Choose $\epsilon>0$.
Since $E_k\in\mathcal{A}_F$, then
$\mu(E_k)=\sup\big\{ \mu(K)\,|\, K\subseteq E_k\;,\; \mbox{\rm $K$ compact}\, \big\}$, hence,
by definition of supremum, there is a compact set
$H_k\subseteq E_k$ such that
\begin{equation}\label{Rudin11}
\mu(H_k)>\mu(E_k)-\frac{\epsilon}{2^{k+1}}\quad (k=1,2,3\cdots)\;.
\end{equation}
Put $K_n:=H_1\cup\cdots\cup H_n$ ($n=1,2,\ldots$).
Clearly, $K_n\subseteq E_1\cup \cdots\cup E_n\subseteq E$,
hence
\begin{equation}\label{Rudin12}
\mu(E)\geq\mu(K_n)=\sum_{k=1}^n\mu(H_k)>\sum_{k=1}^n\mu(E_k)-\frac{\epsilon}{2}\quad (n=1,2,3\cdots)\;,
\end{equation}
where the previous equality is justified by using induction on (\ref{Rudin10}),
taking into account that $H_1,H_2,\ldots,H_n$ are pairwise disjoint compact sets.
Since (\ref{Rudin12}) holds for every $n\in\mathbb{N}$ and $\epsilon>0$, then
sending $n\to\infty$ and $\epsilon\to0$, we obtain $\mu(E)\geq\sum_{k=1}^\infty\mu(E_k)$.
It is clear that the reverse inequality also holds, by Step 1. Thus (\ref{Rudin9}) is proved.

Finally, suppose that $\mu(E)<\infty$. Choose $\epsilon>0$.
By (\ref{Rudin9}), we may ensure the existence of $N=N(\epsilon)\in\mathbb{N}$ such that
\begin{equation}\label{Rudin13}
\mu(E)\leq\sum_{k=1}^N\mu(E_k)+\frac{\epsilon}{2}\; .
\end{equation}
This together with (\ref{Rudin12}) gives $\mu(E)\leq\mu(K_N)+\epsilon$.
We proved that, for every $\epsilon>0$, there exists a compact set
$K\equiv K_N\subseteq E$ such that $\mu(E)\leq\mu(K)+\epsilon$.
By definition of supremum (and taking into account that, by Step 1, $\mu(E)\geq\mu(K)$
for any compact set $K\subseteq E$), this means that
$\mu(E)=\sup\big\{ \mu(K)\,|\, K\subseteq E\;,\; \mbox{\rm $K$ compact}\big\}$,
hence $E\in\mathcal{A}_F$.
\medskip

{\bf Step 5.}
{\it If $E\in\mathcal{A}_F$ and $\epsilon>0$, then
there is a compact set $K$ and an open set $V$ such that}
$$
K\subseteq E\subseteq V\quad\wedge\quad \mu(V-K)<\epsilon\;.
$$

{\it Proof.}
By definition, $\mu(E)$ is given by computing the infimum in (\ref{Rudin2}).
Moreover, being $E\in\mathcal{A}_F$,
$\mu(E)$ is also given by the supremum appearing in the
second condition of the definition of $\mathcal{A}_F$.
Thus, for any $\epsilon>0$, the definitions of infimum and supremum allow us to
find an open set $V\supseteq E$ and a compact set $K\subseteq E$ such that
$$
\mu(V)-\frac{\epsilon}{2}<\mu(E)<\mu(K)+\frac{\epsilon}{2}\;.
$$
This implies $\mu(V)-\mu(K)<\epsilon$.
Since $V-K=V\cap K^c$, then $V-K$ is open (because $K$ is compact, so it is closed, by Theorem \ref{}).
Hence, by Step 3, $V-K\in\mathcal{A}_F$. Also, by Step 2, $K\in\mathcal{A}_F$.
As a consequence, since $V=K\cup(V-K)$, Step 4 implies that
$\mu(V)=\mu(K)+\mu(V-K)$,
hence $\mu(V-K)=\mu(V)-\mu(K)<\epsilon$.
\medskip

{\bf Step 6.}
{\it The following holds:}
$$
A_1,A_2\in\mathcal{A}_F\quad\Rightarrow\quad
A_1-A_2\,,\,A_1\cup A_2\,,\,A_1\cap A_2\in\mathcal{A}_F\;.
$$
%$$
%A,B\in\mathcal{A}_F\quad\Rightarrow\quad
%A-B,A\cup B,A\cap B\in\mathcal{A}_F\;.
%$$
{\it Proof.}
Let $\epsilon>0$. By Step 5, there are compact sets $K_i$ and open sets $V_i$ such that
$$
K_i\subseteq A_i\subseteq V_i\quad\wedge\quad \mu(V_i-K_i)<\epsilon/2\quad (i=1,2)\;.
$$
Since $A_1-A_2\subseteq V_1-K_2\subseteq (V_1-K_1)\cup(K_1-V_2)\cup(V_2-K_2)$, 
by Step 1 we obtain $\mu(A_1-A_2)\leq\mu(V_1-K_1)+\mu(K_1-V_2)+\mu(V_2-K_2)
<\epsilon/2+\mu(K_1-V_2)+\epsilon/2$, hence
\begin{equation}\label{Rudin14}
\mu(A_1-A_2)<\mu(K_1-V_2)+\epsilon\; .
\end{equation}
Taking into account that $A_1\in\mathcal{A}_F$, then $\mu(A_1)<\infty$, 
hence, since $A_1-A_2\subseteq A_1$, we deduce $\mu(A_1-A_2)\leq\mu(A_1)<\infty$.
Moreover, since $K_1-V_2$ is a compact subset of $A_1-A_2$, then (\ref{Rudin14}) shows that
$\mu(A_1-A_2)=\sup\big\{ \mu(K)\,|\, K\subseteq A_1-A_2\;,\; \mbox{\rm $K$ compact}\big\}$.
Therefore, $A_1-A_2\in\mathcal{A}_F$. 
Moreover, since $A_1\cup A_2=(A_1-A_2)\cup A_2$, an application of Step 4 shows that
$A_1\cup A_2\in\mathcal{A}_F$.
Finally, since $A_1\cap A_2=A_1-(A_1-A_2)$, we also have $A_1\cap A_2\in\mathcal{A}_F$.
\medskip

{\bf Step 7.}
{\it $\mathcal{A}$ is a $\sigma-$algebra in $X$ which contains all Borel sets.}
\smallskip

{\it Proof.}
\medskip

{\bf Step 8.}
$\mathcal{A}_F=\{E\in\mathcal{A}\,|\,\mu(E)<\infty\}$.
\smallskip

{\it Proof.}
\medskip

{\bf Step 9.}
{\it $\mu$ is a measure on $\mathcal{A}$.}
\smallskip

{\it Proof.}
The countable additivity of $\mu$ on $\mathcal{A}$ follows immediately by Steps 4 and 8.
\medskip

{\bf Step 10.}
{\it The integral representation} (\ref{repres-Lambda}) {\it holds.}
%{\it For every $f\in\mathcal{C}_0(X)$,}
%\begin{equation}\label{repres-Lambda}
%\Lambda f=\int_{X}f\,{\rm d}\mu\; ,\quad\forall f\in\mathcal{C}_0(X)\;,
%\end{equation}
\smallskip

{\it Proof.}


\qed



\section{Remarks on the Riesz-Markov-Kakutani theorem}

%\section{Remarks and historical notes}




\section*{Exercises}
%\bigskip

%\noindent
\begin{enumerate}[label=\emph{\bf \arabic*.},leftmargin=*]
\item Ex 1
\medskip

%\item
%Sejam $X$ um e.v. real, $p:X\rightarrow\mathbb{R}$ uma funcional sublinear e
%$K:=\{\,x\in X\,|\, p(x)<1\,\}\,$. Mostre que: % $K$ satisfaz as propriedades seguintes:
%\begin{enumerate}
%\item $K$ \'e convexo;
%\item $0$ \'e um ponto interior de $K$ (no sentido da Defini\c c\~ao \ref{def-pontoInt});%(no sentido alg\'ebrico).
%\item $p$ \'e a funcional de Minkowski do conjunto $K$.
%\end{enumerate}
%\medskip

\item
Ex 3
\end{enumerate}
\bigskip

%\medskip

\section*{Bibliography}
%\medskip

{\small
\begin{enumerate}[label=\emph{\rm [\arabic*]},leftmargin=*]
\item\label{Rudin1986} W. Rudin, {\sl Real and Complex Analysis},
          McGraw-Hill (1986) [paperback edition: 2004].
\item\label{EvansGariepy1992} L. Evans, R. Gariepy, {\sl Measure Theory and Fine Properties of Functions},
Studies in Advanced Mathematics, CRC Press (1992).
\end{enumerate}
}


